Efficient Approximation of Certain and Possible Answers for Ranking and Window Queries over Uncertain Data (Extended version)

Uncertainty arises naturally inmany application domains due to, e.g., data entry errors and ambiguity in data cleaning. Prior work in incomplete and probabilistic databases has investigated the semantics and efficient evaluation of ranking and top-k queries over uncertain data. However, most approaches deal with top-k and ranking in isolation and do represent uncertain input data and query results using separate, incompatible datamodels. We present an efficient approach for under- and over-approximating results of ranking, top-k, and window queries over uncertain data. Our approach integrates well with existing techniques for querying uncertain data, is efficient, and is to the best of our knowledge the first to support windowed aggregation. We design algorithms for physical operators for uncertain sorting and windowed aggregation, and implement them in PostgreSQL.We evaluated our approach on synthetic and real world datasets, demonstrating that it outperforms all competitors, and often produces more accurate results.

==> audb-range-windows.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\mypar{Group-based Windowed Aggregation}
Below we formally define for group-based windows for a tuple $\rangeTup$, the certain part of the window $\alwindow{\rangeTup}$ and the possible part of the window $\auwindow{\rangeTup}$. A tuple $\rangeTup'$ belongs certainly to the window for tuple $\rangeTup$, if the ranks it could below too (the interval between the lowest and highest possible rank of the tuple within the partition for $\rangeTup$ is fully contained within the most conservative bounds on ranks for $\rangeTup$, i.e., the greatest possible starting rank and the lowest possible end rank. The multiplicity of $\rangeOf{t'}$ in $\alwindow{\rangeTup}$ is the lowest possible multiplicity for $\rangeOf{t'}$ ($\lbMarker{\rangeRel(\rangeOf{t'})}$). The possible part of the window contains all tuples which may exist and whose interval of possible ranks overlaps with the maximal extend of $\rangeTup$'s window.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure*}[t]
  \centering
  \begin{align*}
    \alwindow{\rangeTup}(\rangeOf{t'}) & =
                                         \begin{cases}
                                           \lbMarker{\alpart{\rangeTup}(\rangeOf{t'})} &\mathif [\lbMarker{\trank{\alpart{\rangeTup}}{\sortattrs}{\rangeOf{t'}}}, \ubMarker{\trank{\alpart{\rangeTup}}{\sortattrs}{\rangeOf{t'}}}]  \\[3mm]
                                                                                       & \subseteq [\ubMarker{\trank{\alpart{\rangeTup}}{\sortattrs}{\rangeTup}} -l, \lbMarker{\trank{\alpart{\rangeTup}}{\sortattrs}{\rangeTup}} + u] \\
                                           0 &\mathotherwise\\
                                         \end{cases}\\
                                         %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \auwindow{\rangeTup}(\rangeOf{t'}) & =
                                         \begin{cases}
                                           \ubMarker{\aupart{\rangeTup}(\rangeOf{t'})} - \alwindow{\rangeTup}(\rangeOf{t'})
                                           &\mathif ([\lbMarker{\trank{\aupart{\rangeTup}}{\sortattrs}{\rangeOf{t'}}}, \ubMarker{\trank{\aupart{\rangeTup}}{\sortattrs}{\rangeOf{t'}}}]  \\
                                           & \cap [\lbMarker{\trank{\aupart{\rangeTup}}{\sortattrs}{\rangeTup}} -l, \ubMarker{\trank{\aupart{\rangeTup}}{\sortattrs}{\rangeTup}} + u]) \neq \emptyset \\
                                           0 &\mathotherwise\\
                                         \end{cases}
                                         % \lbMarker{\rangeOf{P_t} &= \alpart{\rangeTup}
  \end{align*}

  \caption{Certain and possible windows for group-based aggregation over \abbrAUDBs}
  \label{fig:certain-and-poss-group-based-audb-win}
\end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% We exploit this by finding among the tuples that could belong to the window for tuple $\rangeTup$, the tuples with total multiplicity less than or equal to the window size that maximize the aggregation result

% as an \abbrAUDB relation which encodes which tuples belong certainly and possibly to the partition for $\rangeTup$.

% For window function $\omega^{[l,u]}_{f(a) \to x; G; O}$ with preceding parameter $l$, following parameter $u$, aggregation function $f$ over attribute $a$, grouping attributes $G$ and order by attributes $O$, we define ranged window function querying semantics below.

As mentioned before, it would be possible to define aggregation function result bounds based on these definitions alone, but tighter bounds can be achieved if we take into account that each window can contain at most a number of groups that is determined based on the window bounds $[l,u]$. We use $\awinsize$ to denote the size of a window with bounds $[l,u]$, i.e., $\awinsize = l + u + 1$. For that, we combine the certain window (all tuples are that are certainly in the window) with a selected subset of the groups from the possible window that minimizes (for the lower aggregation result bound) or maximizes the (for the upper aggregation result bound) the aggregation function result for an input tuple. Which set of groups that minimizes / maximizes the aggregation result depends on what aggregation function is applied. For \aggmax we do not include any groups from the possible window for the lower bound and the up to $\Kpos$ groups (if this many groups exist) with the largest aggregation input attribute values from the possible window where $\Kpos$ is the size of the window minus the number of tuples that certainly belong to the window. For \aggmin the reverse is true, we only include the $\Kpos$ smallest values for the lower bound and no additional groups for the upper bound. For \aggsum, the $\Kpos$ smallest negative values are included in the lower bound and the $\Kpos$ largest positive values for the upper bound. For \aggcount no additional groups are included for the lower bound and up to $\Kpos$ groups for the upper bound.

\begin{align*}
  \alrestrwin{\rangeTup}{\aggmin}(\rangeOf{t'}.A) &= \lbMarker{\alwindow{\rangeTup}(\rangeOf{t'})} +\\
                                                  &\begin{cases}
                                                    \auwindow{\rangeTup}(\rangeOf{t'}) & \mathif \rangeOf{t'} \in \winbotk{\auwindow{\rangeTup},A,\\
                                                                                     0 & \mathotherwise\\
                                                  \end{cases}\\
  \aurestrwin{\rangeTup}{\aggmin}(\rangeOf{t'}) &= \alwindow{\rangeTup}(\rangeOf{t'})\\[2mm]
\end{align*}


Using the restricted windows we are ready to define group-based windowed aggregation over \abbrUADBs.
In the definition we use $\bgMarker{\rangeRel}$ to denote the select-guess world encoded by $\rangeRel$, i.e., replacing each uncertain attribute value $\uv{c_1}{c_2}{c_3}$ with $c_2$ and tuple annotation $(n_1,n_2,n_3)$ with $n_2$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{Definition}[Group-based Windowed Aggregation]
  Let $\rangeRel$ be an \abbrUADB relation. The group-based window operator $\awinrange$ is defined as shown below.

  \begin{align*}
    \awinrange(\rangeRel)(\rangeTup) &=
    \begin{cases}
      \rangeRel(\rangeOf{t'}) &\mathif \rangeTup = \rangeOf{t'} \tconcat \textendagg{\rangeOf{t'}}{\aggf}{\gbAttrs}{\sortattrs}{l}{u} \\
      0 &\mathotherwise\\
    \end{cases}\\
    \textendagg{\rangeOf{t}}{\aggf}{\gbAttrs}{\sortattrs}{l}{u} &= [\aggf(\alrestrwin{\rangeTup}{\aggf}) / \\ &\hspace{10mm}\aggf(\window{\gbAttrs}{\sortattrs}{l}{u}{\bgMarker{\rangeRel}}{\bgMarker{\rangeTup}}) / \\
    &\hspace{10mm}\aggf(\aurestrwin{\rangeTup}{\aggf})]
  \end{align*}

\end{Definition}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> oldsemwindow.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{Definition}[Ranged window function semantics]
Possible grouping $\ubMarker{P_{t,G}(\rangeRel)}$ and certain grouping $\lbMarker{P_{t,G}(\rangeRel)}$ for tuple $t$ in group by attributes $G$ is defined as:
$$\ubMarker{P_{t,G}(\rangeRel)} = \{ t' \mid t' \in R \land \ubMarker{\seval{t'.G = t.G}{\rval}} \}$$
$$\lbMarker{P_{t,G}(\rangeRel)} = \{ t' \mid t' \in R \land \lbMarker{\seval{t'.G = t.G}{\rval}} \}$$

Upperbound window $\ubMarker{W_{t,G,O,[l,u],a}(\rangeRel)}$ and lowerbound window $\lbMarker{W_{t,G,O,[l,u],a}(\rangeRel)}$ for tuple $t$ group by $G$ order by $O$ with aggregation attribute $a$ is defined as:
\begin{equation*}
\begin{aligned}
	\ubMarker{W_{t,G,O,[l,u],a}(\rangeRel)} & = \\
	\{ t'.a \mid & t' \in \ubMarker{P_{t,G}(\rangeRel)} \land \\
	& (rank(t',O,\rangeRel) \in
	 [\lbMarker{rank(t,O,\rangeRel)} - l, \ubMarker{rank(t,O,\rangeRel)} + u])\ubMarker{}\}
\end{aligned}
\end{equation*}
\begin{equation*}
\begin{aligned}
	\lbMarker{W_{t,G,O,[l,u],a}(\rangeRel)} & = \\
	\{ t'.a \mid & t' \in \lbMarker{P_{t,G}(\rangeRel)} \land \\
	& (rank(t',O,\rangeRel) \in
	 [\ubMarker{rank(t,O,R)} - l, \lbMarker{rank(t,O,\rangeRel)} + u])\lbMarker{}\}
\end{aligned}
\end{equation*}

Upper bound and lower bound on aggregation value is defined as:

\begin{equation*}
\begin{aligned}
\ubMarker{f(W_{t,G,O,[l,u],a}(\rangeRel))} = & f(\{t.a \mid t.a \in \lbMarker{W_{t,G,O,[l,u],a}(\rangeRel)} \lor \\
	 & t.a \in topK(\ubMarker{W_{t,G,O,[l,u],a}(\rangeRel)}) \land t.a > 0 \})
\end{aligned}
\end{equation*}

\begin{equation*}
\begin{aligned}
\lbMarker{f(W_{t,G,O,[l,u],a}(\rangeRel))} = & f(\{t.a \mid t.a \in \lbMarker{W_{t,G,O,[l,u],a}(\rangeRel)} \lor \\
	 & t.a \in botK(\ubMarker{W_{t,G,O,[l,u],a}(\rangeRel)}) \land t.a < 0 \})
\end{aligned}
\end{equation*}

$$K = \mid \lbMarker{W_{t,G,O,[l,u],a}(\rangeRel)} \mid -(l+u)$$

%$$\lbMarker{f(W_{t,G,O,[l,u],a}(R))} = f(\{t.a \mid t.a \in \lbMarker{W_{t,G,O,[l,u],a}(R)} \land t.a < 0 \})$$

The overall window function is defined as:

$$\omega^{[l,u]}_{f(a) \to x; G; O}(\rangeRel) = \{ (t,\ubMarker{f(W_{t,G,O,[l,u],a}(\rangeRel))}, \lbMarker{f(W_{t,G,O,[l,u],a}(\rangeRel))}) \mid t \in \rangeRel \}$$

\end{Definition}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> prob-k-dbs.tex <==
%!TEX root = main.tex
% \subsection{Incomplete K-Relations}
% \label{sec:incompl-prob-k}
% \needRewrite{
% By applying the generalization from~\cite{FH19} called incomplete $\semK$-relations, specifically the $\semN$-relations that model bag-incomplete databases, an incomplete $\semN$-database is a set of $\semN$-databases $\pdb = \{\db_1, \ldots, \db_n\}$  called possible worlds.
% Queries over an incomplete $\semN$-database use
% possible world semantics: The result of a query $\query$ over
% an incomplete $\semN$-database $\pdb$ is the set of possible worlds derived
% by evaluating $\query$ over every world in $\pdb$. 
% }

% %\begin{align*}\label{eq:pqp}
% %\query(\pdb) \defas \comprehension{\query(\db)}{\db \in \pdb} \tag{possible world semantics}
% %\end{align*}
% %

% \iftechreport{
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{Definition} % [Incomplete $\semK$-database]
%   Let $\semK$ be a semiring. An \emph{incomplete $\semK$-database} $\pdb$ is a set of $\semK$-databases $\pdb = \{\db_1, \ldots, \db_n\}$   called possible worlds.
% \end{Definition}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% % Like classical incomplete databases,
% Queries over an incomplete $\semK$-database use
% possible world semantics, i.e., the result of evaluating a query $\query$ over
% an incomplete $\semK$-database $\pdb$ is the set of all possible worlds derived
% by evaluating $\query$ over every possible world $\db \in \pdb$.
%  % The only difference is that $\semK$-relational query semantics is used.
% %
% \begin{align}\label{eq:pqp}
% \query(\pdb) \defas \comprehension{\query(\db)}{\db \in \pdb}
% \end{align}
% %
% }
% \needRewrite{
% Generalizing certain and possible answers,
% %   For incomplete $\semN$-relations, the certain and possible multiplicities of tuples are used as a generalization of certain and possible answers. % For semiring $\semN$,
% % The
% the certain (possible)
% multiplicity % $\pwCertainN(\pdb, \tup)$ ($\pwPossibleN(\pdb, \tup)$)
% of a tuple $\tup$ in an incomplete $\semN$-database $\pdb$ is % defined as
% the minimum (maximum) multiplicity of the tuple across all possible worlds:\\[-10mm] }
% \begin{center}
%   \begin{align*}
%   %  \pwCertain(\setK) &= \GlbK(\setK)
%                          \pwCertainN(\pdb,\tup)  &\defas \min(\{\db(\tup) \mid \db \in \pdb \})\\
% \pwPossibleN(\pdb,\tup) &\defas \max(\{\db(\tup) \mid \db \in \pdb \})
%   \end{align*}
% \end{center}

\iftechreport{
%(i.e., $\query(\pdb) = \{ \query(\db_1), \ldots, \query(\db_n) \}$).

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Certain and Possible Annotations} %Answers}
\label{sec:poss-worlds-cert}

For incomplete $\semK$-relations, we define the certain and possible annotations of tuples as a generalization of certain and possible answers in classical incomplete databases. For these concepts to be well-defined we require that $\semK$ is an l-semiring~\cite{DBLP:conf/icdt/KostylevB12} which means that the natural order forms a lattice. Most commonly considered semirings (e.g., sets, bags, most provenance semirings, \ldots) are l-semirings.
The \emph{certain annotation} of a tuple, is the greatest lower bound (\emph{glb}) of its annotations across all possible world while the \emph{possible annotation} is the least upper bound (\emph{lub}) of these annotations.
We use $\glbK$ (glb) and $\lubK$ (lub)
to denote the $\glb$ and $\lub$
operations for a semiring $\semK$.
The certain (possible)
annotation $\pwCertain(\pdb, \tup)$ ($\pwPossible(\pdb, \tup)$) of a tuple $\tup$ in an incomplete $\semK$-database $\pdb$ is defined as the glb (lub) over the annotations of tuple $\tup$ across all possible worlds of $\pdb$: % of this set.
%\\[-8mm] % respectively.
%
\begin{center}
  \begin{align*}
  %  \pwCertain(\setK) &= \GlbK(\setK)
                         \pwCertain(\pdb,\tup)  &\defas \GlbK(\{\db(\tup) \mid \db \in \pdb \})\\
\pwPossible(\pdb,\tup) &\defas \lubK(\{\db(\tup) \mid \db \in \pdb \})
  \end{align*}
\end{center}
Importantly, this coincides with the standard definition of certain and possible answers for set semantics ($\semB$): the natural order of the set semiring $\semB$ is $\bfalse \ordOf{\semB} \btrue$, $k_1 \lubKof{\semB} k_2 = k_1 \vee k_2$,  % and $k_1
and $k_1 \glbKof{\semB} k_2 = k_1 \wedge k_2$. That is, a tuple is certain (has certain annotation $\btrue$) if it exists (is annotated with $\btrue$) in every possible world and possible if it exists in at least one possible world (is annotated with $true$ in one or more worlds). The natural order of $\semN$ is the standard order of natural numbers. We get  $\pwCertOf{\semN} = \min$ and $\pwPossOf{\semN} = \max$.
This coincides with % Guagliardo and Libkin's
the definition of certain and possible multiplicity for bag semantics from~\cite{GL16,CG19,DBLP:conf/pods/ConsoleGLT20}. % which defines
}
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> semirings.tex <==
%!TEX root = main.tex
\subsection{K-Relations} \label{sec:data_provenance}
\needRewrite{
The generalization of incomplete databases we use here is based on  \textbf{$\semK$-relations}~\cite{Green:2007:PS:1265530.1265535}. 
%$\semK$-relations is a generalization of classical incomplete databases called incomplete $\semK$-relations. 
In this framework, relations are annotated with elements from the domain $\kDom$ of a (commutative) semiring $\semK=\tuple{\kDom,\addK,\multK,\oneK,\zeroK}$, i.e., a mathematical structure with commutative and associative addition ($\addK$) and product ($\multK$) operations where $\addK$ distributes over $\multK$ and $k \multK \zeroK = \zeroK$ for all $k \in K$.
An $n$-nary $\semK$-relation is a function that maps tuples % (elements from $\aDom^{n}$)
to elements from $\kDom$.
Tuples that are not in the relation are annotated with $\zeroK$. %, then this tuple is not in the relation.
%If $\aDom$ is infinite, then it is additionally required that
Only finitely many tuples may be mapped to an element other than $\zeroK$. % (i.e., relations must be finite).
Since $\semK$-relations are functions from tuples to annotations, it is customary to denote the annotation of a tuple $\tup$ in relation $\rela$ as $\rela(\tup)$. }

% (applying function $\rela$ to input $\tup$).
% The specific information encoded by an annotation % other than $\zeroK$
%  depends on the choice of semiring.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\mypar{Encoding Sets and Bags}
%Green et al.~\cite{Green:2007:PS:1265530.1265535} demonstrated that
% \ifnottechreport{
%   In this work we are interested in bag semantics, which can be encoded using the semiring of natural numbers with standard addition and multiplication $\tuple{\semN, +, \times, 0, 1}$ to annotate each tuple with its multiplicity. % For the remainder of this paper we limit the discussion to this semiring.
%   We discuss the applicability of our framework to a larger class of semirings in an accompanying technical report~\cite{techreport}. % with the exception of a brief discussion of the applicability of our results to other semirings in \Cref{sec:conclusions}. %
%}
%\iftechreport{
%The specific information encoded by an annotation % other than $\zeroK$
% depends on the choice of semiring.
%  For instance, bag and set relations can be encoded as
% semirings: the natural numbers ($\semN$) with addition and multiplication, $\tuple{\semN, +, \times, 0, 1}$, annotates each tuple with its multiplicity; and boolean constants $\semB = \{T,F\}$ with disjunction and conjunction, $\tuple{\semB, \vee, \wedge, F, T}$, annotates each tuple with its set membership.
% Abusing notation, we often use $\semK$ to denote both the domain and the corresponding semiring.
% }

 \ifnottechreport{
 % \mypar{Query Semantics}
Operators of positive relational algebra ($\raPlus$) over $\semN$-relations % are defined by
combine input annotations using % operations
$\addN$ and $\multN$. % operations of the semiring as follows:
%
\begin{align*}
	\textbf{Union: } & (R_1 \union R_2)(t) = R_1(t) \addN R_2(t) \\
	\textbf{Join: } & (R_1 \join R_2)(t) = R_1(t[{\schemaOf(\rela_1}) ]) \multN R_2(t[{\schemaOf(\rela_2}) ]) \\
  \textbf{Projection: } & (\projection_U (R))(t) = \sum_{t=t'[U]}R(t')\\
  \textbf{Selection: } & (\selection_\theta(R))(t) = R(t) \multN \theta(t)
\end{align*}
   }
\iftechreport{

\mypar{Query Semantics}
Operators of the positive relational algebra ($\raPlus$) over $\semK$-relations are defined by combining input annotations using operations $\addK$ and $\multK$. % operations of the semiring as follows:
%

\begin{align*}
	\textbf{Union: } & (R_1 \union R_2)(t) = R_1(t) \addK R_2(t) \\
	\textbf{Join: } & (R_1 \join R_2)(t) = R_1(t[\relschema_1 ]) \multK R_2(t[\relschema_2 ]) \\
  \textbf{Projection: } & (\projection_U (R))(t) = \sum_{t=t'[U]}R(t')\\
  \textbf{Selection: } & (\selection_\theta(R))(t) = R(t) \multK \theta(t)
\end{align*}
}
\iftechreport{
For simplicity we assume in the definition above that tuples are of a compatible schema (e.g., $\relschema_1$ for a union $R_1 \union R_2$).
We use $\theta(t)$ to denote a function that returns $\oneK$ iff $\theta$ evaluates to true over tuple $t$ and $\zeroK$ otherwise.
}
\iftechreport{
A \textbf{homomorphism} is a mapping $h: \semK \to \semK'$ from a semiring $\semK$ to a semiring $\semK'$ that maps $\zeroOf{\semK}$ and $\oneOf{\semK}$ to their counterparts in $\semK'$ and distributes over sum and product (e.g., $h(k \addK k') = h(k) \addOf{\semK'} h(k')$).
Any homomorphisms $h$ can be lifted from semirings to $\semK$-relations or $\semK$-databases  by applying $h$ to the annotation of every tuple $\tup$: $h(R)(t) = h(R(t))$. We will use the same symbol for a homomorphism and its lifted variants.
Importantly, queries commute with semiring homomorphisms: $h(\query(\db)) = \query(h(\db))$.
}
We will make use of the so called \textit{natural order} $\ordK$ for a semiring $\semK$
which is the standard order $\leq$ of natural numbers for $\semN$.
\iftechreport{
Formally, $k \ordK k'$ if it is possible to obtain $k'$ by adding to $k$: $\exists k'': k \addK k'' = k'$. % some value $k''$ to $k$.
Semirings for which the natural order is a partial order are called \textit{naturally ordered}~\cite{Geerts:2010bz}.
\begin{align}
\forall k, k' \in \kDom: \big(k \ordK k'\big) \Leftrightarrow \big(\exists k'' \in \kDom: k \addK k'' = k'\big)
\end{align}
}
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> ua-rels.tex <==
%!TEX root = ./main.tex
% -*- root: main.tex -*-
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{AU-Databases} \label{sec:AU-model}

Using $\semK$-relations and \abbrUADBs, Feng et al.~\cite{FH19} introduced \textit{\abbrAUDBs} (\textit{attribute-annotated uncertain databases}) which is a special type of $\semK$-relation over \textit{range-annotated domains}. Encodes attribute and tuple level under- and over-\-ap\-prox\-i\-ma\-tion of the certain and possible multiplicity of tuples from an incomplete $\semN$-database $\pdb$ (bag semantics).
\BGI{Needs a bit introduction what the purpose of these range-annotated values is (compact encoding of many possibilities / attribute-level uncertainty)}
In a \abbrAUDB, a value is called \textit{range-annotated value} $c = \uv{\lbMarker{c}}{\bgMarker{c}}{\ubMarker{c}}$ from a \textit{range-annotated domain} $\rangeDom$ encodes a value $\bgMarker{c} \in \dataDomain$ and two values ($\lbMarker{c}$ and $\ubMarker{c}$) that bound $\bgMarker{c}$ from below and above. We call a value $c \in \rangeDom$ certain if $\lbMarker{c}=\bgMarker{c}=\ubMarker{c}$.
For any $c \in \rangeDom$ we have $\lbMarker{c} \leq \bgMarker{c} \leq \ubMarker{c}$. For each tuple, \abbrUAADBs use $\semqN = \tuple{\semqN, \addOf{\semqN}, \multOf{\semqN}, \zeroOf{\semqN}, \oneOf{\semqN}}$ annotations to encode $\ut{\lbMarker{k}}{\bgMarker{k}}{\ubMarker{k}}$: a lower bound on the certain multiplicity of the tuple, the multiplicity of the tuple in the \abbrBGW, and an over-approximation of the tuple's possible multiplicity.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{\abbrAUDB Expression evaluation}
  Let $\sexpr$ be an expression. Given a range valuation $\rval: \vars(e) \rightarrow \rangeDom$,
selected guess expression evaluation is defined as % $\bgMarker{\rval}$ as the valuation
$\bgMarker{\rval}(x) \defas \bgMarker{\rval(x)}$.
  The result of expression $\sexpr$ over $\rval$ denoted as $\seval{\sexpr}{\rval}$ is defined as:
    \begin{align*}
      \seval{x}{\rval} &\defas \uv{\lbMarker{\rval(x)}}{\bgMarker{\rval(x)}}{\ubMarker{\rval(x)}} &
      \seval{c}{\rval} &\defas \uv{c}{c}{c}
    \end{align*}
    \ifnottechreport{
    Selected guess\BG{?} For any of the following expressions is defined as $\bgMarker{\seval{e}{\rval}} \defas \seval{e}{\bgMarker{\rval}}$. Let $\seval{e_1}{\rval} = a$, $\seval{e_2}{\rval} = b$, and $\seval{e_3}{\rval} = c$. All expressions omitted below are defined point-wise (e.g., $\lbMarker{\seval{e_1 + e_2}{\rval}} \defas \lbMarker{a} + \lbMarker{b}$).\BGI{We can see later which of these operations we need and just refer to the previous paper for the others}
%
   \begin{align*}
%%%%%%%%%%%%%%%%%%%%
% 	 \lbMarker{\seval{e_1 \wedge e_2}{\rval}} &\defas \lbMarker{a} \wedge \lbMarker{b} &
% 	 \ubMarker{\seval{e_1 \wedge e_2}{\rval}} &\defas \ubMarker{a} \wedge \ubMarker{b}\\
% %%%%%%%%%%%%%%%%%%%%
%       \lbMarker{\seval{e_1 \vee e_2}{\rval}} &\defas \lbMarker{a} \vee \lbMarker{b} &
%       \ubMarker{\seval{e_1 \vee e_2}{\rval}} &\defas \ubMarker{a} \vee \ubMarker{b} \\
%%%%%%%%%%%%%%%%%%%%
      \lbMarker{\seval{\neg e_1}{\rval}} &\defas \neg\, \ubMarker{a} &
      \ubMarker{\seval{\neg e_1}{\rval}} &\defas \neg\, \lbMarker{a}
%%%%%%%%%%%%%%%%%%%%
      % \lbMarker{\seval{e_1 + e_2}{\rval}} &\defas \lbMarker{a} + \lbMarker{b} &
      % \ubMarker{\seval{e_1 + e_2}{\rval}} &\defas \ubMarker{a} + \ubMarker{b}
    \end{align*}\\[-10mm]
    \begin{align*}
%%%%%%%%%%%%%%%%%%%%
      \lbMarker{\seval{e_1 \cdot e_2}{\rval}}                                                                                         &\defas \min(\;\;\ubMarker{a} \cdot \ubMarker{b},\;\;
                      \ubMarker{a} \cdot \lbMarker{b},\;\;
                      \lbMarker{a} \cdot \ubMarker{b},\;\;
                      \lbMarker{a} \cdot \lbMarker{b}\;\;)\\
      \ubMarker{\seval{e_1 \cdot e_2}{\rval}}                                                                       &
      \defas \max(\;\;\ubMarker{a} \cdot \ubMarker{b},\;\;
                      \ubMarker{a} \cdot \lbMarker{b},\;\;
                      \lbMarker{a} \cdot \ubMarker{b},\;\;
                      \lbMarker{a} \cdot \lbMarker{b}\;\;)
     %%%%%%%%%%%%%%%%%%%%
    \end{align*}\\[-10mm]
    \begin{align*}
      \lbMarker{\seval{e_1 \leq e_2}{\rval}} &\defas \ubMarker{a} \leq \lbMarker{b} &
 \lbMarker{\seval{e_1=e_2}{\rval}} &\defas \ubMarker{a}=\lbMarker{b} \wedge \ubMarker{b}=\lbMarker{a} \\
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 \ubMarker{\seval{e_1 \leq e_2}{\rval}} &\defas \lbMarker{a} \leq \ubMarker{b} &
                                                                                                 \ubMarker{\seval{e_1=e_2}{\rval}} &\defas \lbMarker{a} \leq \ubMarker{b} \wedge \lbMarker{b} \leq \ubMarker{a}
 % \ubMarker{a}>\lbMarker{b} \wedge \lbMarker{a}<\lbMarker{b} \vee \ubMarker{a}>\ubMarker{b} \wedge \lbMarker{a}<\ubMarker{b} \\
    \end{align*}\\[-10mm]
    \begin{align*}
\lbMarker{\seval{\ifte{e_1}{e_2}{e_3}}{\rval}} &\defas
 \begin{cases}
\lbMarker{b} & \text{if } \lbMarker{a}= \ubMarker{a}=\btrue \\
\lbMarker{c} & \text{if } \lbMarker{a}= \ubMarker{a}=\bfalse \\
 \min(\lbMarker{b},\lbMarker{c}) & \text{else}
\end{cases}\\
      \ubMarker{\seval{\ifte{e_1}{e_2}{e_3}}{\rval}} &\defas
 \begin{cases}
 \ubMarker{b} & \text{if } \lbMarker{a}= \ubMarker{a}=\btrue \\
\ubMarker{c} & \text{if } \lbMarker{a}= \ubMarker{a}=\bfalse \\
\max(\ubMarker{b},\ubMarker{c}) & \text{else}
\end{cases}
    \end{align*}
    }
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsubsection{Aggregation monoids}
\abbrAUDB use commutative monoids~\cite{amsterdamer2011provenance} $\tuple{\monoid, \amadd, \amzero}$ to define $\semK$-relations aggregation semantics for aggregation functions. Values from commutative monoids $\monoid$ are the input to aggregation that combined through operation $\amadd$ with a neutral element $\amzero$. Consider a monoid $\monoid \in \{\msum, \mmin, \mmax\}$. % such that $\smbN{\monoid}$ is well defined.
  Let $\uv{\lbMarker{m}}{m}{\ubMarker{m}}$ be a range-annotated value from $\rangeDom$ and $\ut{\lbMarker{k}}{k}{\ubMarker{k}} \in \uaaK{\semN}$.
  %Let triple  that  the value domain. Let triple $\semNX^3=(\lbMarker{x},x,\ubMarker{x})$ denote a tuple annotation value in \abbrAUDB.
Monoid over range annotated domain is defined as $\ut{\lbMarker{k}}{k}{\ubMarker{k}} \amysmbNAU \uv{\lbMarker{m}}{m}{\ubMarker{m}} =$
%  We define $\amysmbNAU$ as shown below. % range aggregation monoid multiplication computation yields a triple as below.
  % \begin{flalign*}
  %     \ut{\lbMarker{k}}{k}{\ubMarker{k}} \amysmbNAU \uv{\lbMarker{m}}{m}{\ubMarker{m}} =
  % \end{flalign*}
%%%%%%%%%%%%%%%%%%%%
  \begin{align*}
		[& min(\lbMarker{k} \smbN{\monoid} \lbMarker{m},\lbMarker{k} \smbN{\monoid} \ubMarker{m},\ubMarker{k} \smbN{\monoid} \lbMarker{m},\ubMarker{k} \smbN{\monoid} \ubMarker{m}), \\
		& {k} \smbN{\monoid} {m}, \\
		& max(\lbMarker{k} \smbN{\monoid} \lbMarker{m},\lbMarker{k} \smbN{\monoid} \ubMarker{m},\ubMarker{k} \smbN{\monoid} \lbMarker{m},\ubMarker{k} \smbN{\monoid} \ubMarker{m})]
	\end{align*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

    \subsubsection{\abbrAUDB Aggregation}
    In order to define uncertain window functions, we base on some notations from \abbrAUDB aggregations. Different from aggregations, uncertain window functions intuitively have an uncertain group for each tuple and compute aggregation results on each group individually which is a different group strategy.
    \BGI{This requires some more explanations and we should start by stating why the reader needs to understand AU-DB aggregation (because we need it for window functions)}
\abbrAUDB aggregation semantics first define a grouping strategy for each group.
\begin{align*}
 \gsdefG(\gbAttrs, \rangeRel)                      & \defas  \{ t.\gbAttrs \mid \exists \rangeTup: \bgMarker{\rangeTup} = t \wedge \rangeRel(\rangeTup) \neq \uaaZero{\semN} \} &
  % \gsdefBG(\rangeTup')        & \defas \bgMarker{\rangeTup'.\gbAttrs}  &
  \gsdefP(\rangeTup)          & \defas \bgMarker{\rangeTup.\gbAttrs}
\end{align*}
Then bounds for group by attribute values are defined as:
\begin{align*}
\lbMarker{\aout.a} &= \min_{\rangeTup: \stratPoss(\rangeTup) = \asgrp} \lbMarker{\rangeTup.a} &
\bgMarker{\aout.a} &= \agroup.a &
\ubMarker{\aout.a} &= \max_{\rangeTup: \stratPoss(\rangeTup) = \asgrp} \ubMarker{\rangeTup.a}
\end{align*}
Then the aggregation function result bounds are defined as:
\begin{align*}
    \tgrouping(\asgrp) \defas \{ \rangeTup \mid \rangeRel(\rangeTup) \neq \uaaZero{\semN} \wedge \rangeTup.\gbAttrs \toverlaps \aout.\gbAttrs\}
  \end{align*}
  %%%%%%%%%%%%%%%%%%%%
  The aggregation function result bounds for tuple $\aout$ are defined as: \\[-3mm]
  %%%%%%%%%%%%%%%%%%%%
  \begin{align*}
    \lbMarker{\aout.f(A)} &= \sum_{\rangeTup \in \tgrouping(\asgrp)} \lbagg{\rangeTup}
  &\ubMarker{\aout.f(A)} &= \sum_{\rangeTup \in \tgrouping(\asgrp)} \ubagg{\rangeTup}
  \end{align*}\\[-6mm]
  \begin{align*}
     \bgMarker{\aout.f(A)} &= \sum_{\rangeTup \in \tgrouping(\asgrp)} \bgMarker{(\rangeRel(\rangeTup) \amysmbNAU \rangeTup.A)}
  \end{align*}\\[-6mm]
  %%%%%%%%%%%%%%%%%%%%
  \begin{align*}
  \lbagg{\rangeTup}     &= \begin{cases}
                            min(\amzero,\lbMarker{(\rangeRel(\rangeTup) \amysmbNAU \rangeTup.A)}) &\mathtext{if }\uncertg{\gbAttrs}{\rangeRel}{\rangeTup} \\
                            \lbMarker{(\rangeRel(\rangeTup) \amysmbNAU \rangeTup.A)} &\mathtext{otherwise}\\
                          \end{cases}\\
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \ubagg{\rangeTup}     &= \begin{cases}
                            max(\amzero,\ubMarker{(\rangeRel(\rangeTup) \amysmbNAU \rangeTup.A)}) &\mathtext{if }\uncertg{\gbAttrs}{\rangeRel}{\rangeTup} \\
                            \ubMarker{(\rangeRel(\rangeTup) \amysmbNAU \rangeTup.A)}&\mathtext{otherwise}\\
                          \end{cases} \\
  \uncertg{\gbAttrs}{\rangeRel}{\rangeTup} & \defas (\exists a \in \gbAttrs: \lbMarker{\rangeTup.a} \neq \ubMarker{\rangeTup.a}) \vee \lbMarker{\rangeRel(\rangeTup)} = 0 \\
  \rangeTup \toverlaps \rangeTup' & \defas \bigwedge_{i \in \{1, \ldots, n\}} [ \lbMarker{\rangeTup.A_i}, \ubMarker{\rangeTup.A_i} ] \cap  [ \lbMarker{\rangeTup'.A_i}, \ubMarker{\rangeTup'.A_i} ] \neq \emptyset
\end{align*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{\needRewrite{Preservation of bounds}}

\BGI{Add brief description of the main result from the AU-DB paper and what it means. We should probably define bound-preservation and bounding since we need to prove it for the ranking / window semantics.}
\abbrUAADB define what it means to bound an incomplete $\semN$-relation by first define bounding of deterministic tuples by range-annotated tuples. % bound (match).
%We use \abbrUAADB relation to bound all possible worlds from an incomplete database. Starting from bounding a tuple from each possible world to a \abbrUAADB tuple.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%\begin{Definition}% [Tuple Bounding]
  %%\label{def:bounding-tuples}
  Let  $\rangeTup$ be a  range-annotated tuple with schema $\tuple{a_1, \ldots, a_n}$ and   $\tup$ be a tuple  with the same schema as $\rangeTup$. We say that $\rangeTup$ bounds $\tup$ written as $\tup \tmatch \rangeTup$ iff\\[-3mm]
  %

  \[
    \forall{i \in \{1, \ldots ,n\}}:
    \lbMarker{\rangeTup.a_i} \leq \tup.a_i \leq \ubMarker{\rangeTup.a_i}
  \]
%%\end{Definition}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{Definition}[Bounding $\uaaN$ Annotations]\label{def:bounding-annotations}
% 	A value $k \in \uaaN$ is said to bound a set of values $S_k = \{k_1, \ldots, k_n\}$ from $\semN$ if:
%   \begin{align*}
%     \forall k_i \in S_k: \lbMarker{k} \leq k_i \leq \ubMarker{k}\\
%     \exists k_i \in S_k: k_i = \bgMarker{k}
%   \end{align*}
% \end{Definition}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
One \abbrUAADB tuple may bound multiple conventional tuples and vice versa. We define \textit{tuple matchings} as a way to match the multiplicities of  tuples of a $\uaaN$-database (or relation) with that of one possible world of an incomplete $\semN$-database (or relation).
Based on tuple matchings we then define how to  bound possible worlds.
% a mapping between a set of \abbrUAADB tuples and a set of deterministic tuples.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%\begin{Definition}% [Tuple matching]
  %%\label{def:tuple-matching}
  Let $\rangeRel$ be an $n$-ary \abbrUAARel and $\rela$ an $n$-ary relation. A \emph{tuple matching} $\TM$ for $\rangeRel$ and $\rela$ is a function $(\rangeDom)^{n} \times \dataDomain^n \to \semN$.
  % $$TM_{R^I,R}(\rangeTup,t)=k$$ is the mappings from an annotated tuple $\rangeTup$ and a possible world tuple $t$ to a semiring element $k$
  \st the following conditions hold:\\[-3mm]

  %%%%%%%%%%%%%%%%%%%%
  \begin{align*}
    &\forall \rangeTup \in \rangeDom^n: \forall \tup \ntmatch \rangeTup: \TM(\rangeTup, \tup) = \zeroN
    &\forall \tup \in \dataDomain^n: \hspace*{-1mm}\sum_{\rangeTup \in \rangeDom^n} \hspace*{-1mm}\TM(\rangeTup, \tup)=\rela(\tup)
  \end{align*}
%%\end{Definition}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

A tuple matching distributes the multiplicity of a tuple from $\rela$ over one or more matching tuples from $\rangeRel$.  Multiple tuples from an \abbrUAADB may encode the same tuple when the multidimensional rectangles of their attribute-level range annotations overlap, as with the first two tuples of the \abbrUAADB in \Cref{table:UAAR_overall} and the \abbrBGW.
%. For instance,  $\tuple{\uv{1}{2}{3}}$ and $\tuple{\uv{2}{3}{5}}$ both match the tuple $\tuple{2}$.
% The conditions stating that a \abbrUAADB tuple can only match to conventional tuple if the tuple is bounded by the \abbrUAADB tuple. Also all the conventional tuples in relation $\rela$ need to be matched in the tuple matching.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%\begin{Definition}\label{def:bounding-worlds}
  Given an n-ary \abbrUAADB relation $\rangeRel$ and an n-ary deterministic $\semN$-relation $\rela$ (a possible world),  relation $\rangeRel$ bounds $\rela$ (denoted $\rela \dbbounds \rangeRel$) iff there exists a tuple matching $\TM$ for $\rangeRel$ and $\rela$ \st \\[-5mm]
%
  \begin{align*} %\label{eq:lower-bound-db}
    &\forall \rangeTup \in \rangeDom^n:\sum_{\tup \in \dataDomain^n} \TM(\rangeTup,\tup) \geq \lbMarker{\rangeRel(\rangeTup)}
    \;\text{\textbf{and}}\; % \forall \rangeTup \in \rangeDom^n:
       \sum_{\tup \in \dataDomain^n} \TM(\rangeTup,\tup) \leq \ubMarker{\rangeRel(\rangeTup)} %\label{eq:upper-bound-db}
  \end{align*}
%%\end{Definition}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Having defined when a possible world is bound by a $\uaaN$-relation, we are ready to define bounding of incomplete $\semN$-relations.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	Given an incomplete $\semN$-relation $\prel$ and a $\uaaN$-relation $\rangeRel$, we say that $\rangeRel$ bounds $\prel$, written as $\prel \dbbounds \rangeRel$
  iff
    \begin{align*}
    &\forall \rela \in \prel: \rela \dbbounds \rangeRel
    &&\exists \rela \in \prel: \rela = \bgOf{\rangeRel}
    \end{align*}

\abbrAUDB querying semantics is defined and closed under $\raPlus$, Set difference and aggregations. \abbrAUDB also proved bound preservation on all operations.


\subsubsection{Relational encodings}
\abbrAUDB can be encoded in a relational database by encoding domain values in triple columns each encodes the lower bound, best guess and upper bound value.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> uaa-aggregation.tex <==
%!TEX root=./uaadb.tex
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Aggregation}\label{sec:aggregation}

We now introduce a bound preserving semantics for aggregation over $\uaaN$-relations
that is based on results from~\cite{amsterdamer2011provenance} that we review below.We leave a generalization to other semirings to future work. See~\cite{techreport} for a discussion of the challenges involved with that. Importantly, our semantics has \ptime data complexity.
% The semantics of~\cite{amsterdamer2011provenance}
% % One major challenge in defining aggregation over $\semK$-relations
% % which also applies to our problem setting is that one has to
% takes tuple annotations into account when calculating aggregation function
% results. For instance, under bag semantics (semiring $\semN$) the multiplicity
% of a tuple affects the result of $\aggsum$ aggregation.
% However, additional complications arise for $\uaaN$-relations, because the techniques from~\cite{amsterdamer2011provenance} are not directly applicable and we have to deal with uncertain group memberships.


% of tuples across possible worlds.
% For \abbrUAADBs we have to overcome two major new challenges: (i)
% since the values of group-by attributes may be uncertain, a tuple's group
% membership may be uncertain too and (ii) we are aggregating over range-bounded
% values.
% To address (ii) we  utilitze our expression semantics for
% range-bounded values from \Cref{sec:expression}. However, additional
% complications arise when taking the $\uaaK{\semN}$-annotations of tuples into
% account. For (i) we will reason about all possible group memberships of
% range-annotated tuples to calculate bounds on group-by values, aggregation
% function results, and number of result groups.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{Background}
% \label{sec:background-1}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\mypar{Aggregation Monoids}
%
The semantics for aggregation queries
over $\semK$-relations from~\cite{amsterdamer2011provenance} deals with aggregation functions that
are commutative monoids $\tuple{\monoid, \amadd, \amzero}$, i.e., where
the values from
$\monoid$ that are the input to aggregation are combined through an operation
$\amadd$ which has a neutral element $\amzero$. Abusing notation, we will use $\monoid$ to both denote the monoid and its domain.
% \footnote{A monoid is a
  % mathematical structure $(\monoid, \amadd, \amzero)$ where $\amadd$ is a
  % commutative and associative binary operation over $\monoid$, and $\amzero$ is
  % the neutral element of $\monoid$. For instance,
  % $\msum \defas (\mathbb{R}, +, 0)$, i.e., addition over the reals can be used
  % for sum aggregation.}
Standard aggregation functions \aggsum, \aggmin, \aggmax, and \aggcount are
monoids. \aggavg can be derived from \aggsum and \aggcount. % (\msum and
% \aggsum).
As an example, consider the monoids for $\aggsum$ and $\aggmin$:
$\msum \defas \tuple{\mathbb{R}, +, 0}$ and $\mmin \defas \tuple{\mathbb{R}, \min,
\infty}$.
%The result of aggregation over a set of $\monoid$ values is defined as the sum of these values in  $\monoid$.
For $\monoid \in \{\msum, \mmin, \mmax\}$ (\aggcount uses \msum), we define a corresponding monoid  $\rangeMon$ using
range-annotated expression semantics (\Cref{sec:expression}). Note that this gives us aggregation functions which can be applied to range-annotated values and are bound preserving, i.e., the result of the aggregation function bounds all possible results for any set of values bound by the inputs.
For example, $\aggmin$ is expressed as $\min(v,w) \defas \ifte{v \leq w}{v}{w}$.
% we can define  $\monoid$
% ($\msum$)
% Note that bound-preserving evaluation of these monoids over
% range-annotated values is already supported though the range-annotated
% expression semantics from \Cref{sec:expression}.
% For instance, $\msum$ simply
%uses the addition operation we defined.
% Even though we did not define $\aggmin$
% and $\aggmax$ explicitly, we can express them using the operators
%  from~\Cref{sec:expression}, e.g., $\min(v,w) \defas \ifte{v \leq w}{v}{w}$. In
%  the following, we use $\rangeMon$ to denote the range-annotated version of
%  $\monoid$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{Lemma}\label{lem:range-annotated-monoids}
$\rangeMof{\msum}$, $\rangeMof{\mmin}$, $\rangeMof{\mmax}$ are monoids.
\end{Lemma}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{proof}[Proof Sketch]
  Proven by unfolding of definitions to show that the addition operations of these monoids is  pointwise application of the operation of the monoids they originated from.
\end{proof}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Based on \Cref{lem:range-annotated-monoids} we have that aggregation functions
% over range-annotated values preserve bounds.

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{figure}[t]
%   \centering
%   \begin{align}
%     k \smbN{\monoid} (m_1 \amadd m_2) & = k \smbN{\monoid} m_1 \amadd k \smbN{\monoid} m_2 \label{eq:semimodule-distributes-over-m-plus}\\
%     % (k_1 \addN k_2) \smbN{\monoid} m  & = k_1 \smbN{\monoid} m \amadd k_2 \smbN{\monoid} m \\
%     % \oneN \smbN{\monoid} m            & = m                                                    \\
%     % \zeroN \smbN{\monoid} m           & = \amzero            \label{eq:semimodule-with-m-zero-yields-m-zero}                                  \\
%     k \smbN{\monoid} \amzero          & = \amzero                                              %\\
%     % (k_1 \multN k_2) \smbN{\monoid} m & = k_1 \smbN{\monoid} (k_2 \smbN{\monoid} m)
%   \end{align}\\[-3mm]
%   \caption{Semimodule laws excerpt (semiring $\semN$, monoid $\monoid$)}
%   \label{fig:semimodule-laws}
% \end{figure}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\mypar{Semimodules}
%
Aggregation over
$\semK$-relations  has to take the annotations of tuples into account for computing
aggregation results. For instance, consider an $\semN$-relation $R(A)$ with
tuples $\tuple{30} \mapsto 2$ and $\tuple{40} \mapsto 3$, (i.e., respectively 2 and 3 duplicates).
The sum over $A$ should be $30 \cdot 2 + 40 \cdot 3 = 180$.
More generally speaking, we
need an operation $\smbpair_{\monoid}: \semN \times \monoid \rightarrow \monoid$
that combines the tuple multiplicities with domain values.
As observed in~\cite{amsterdamer2011provenance}
this operation has to fulfill the algebraic laws of semimodules. %, i.e., it has to fulfill a set of algebraic laws. % , two of which are shown for $\semN$ in \Cref{fig:semimodule-laws}.
% \BGdel{Note that in the example above we made use of the fact that
% $\smbN{\msum}$ is $\cdot$ to get
% $30 \smbN{\msum} 2 = 30 \cdot 2 = 60$.}
% In the following, we will use $\smbpair_{\monoid}$ to denote $\smbN{\monoid}$.
Note that  $\smbpair$ is  well-defined % for
% all semirings, but it is defined
for $\semN$ and all of the monoids we consider:\\[-6mm]
% We discuss the general case in \cite{techreport}.
%We show the definition for $\smbN{\monoid}$ for all considered monoids below:
%
\begin{align*}
  k \smbN{\msum} m                        & = k \cdot m             &
  k \smbN{\mmin} m = k \smbN{\mmax} m & =
  \begin{cases}
    m                                         & \text{if}\,\,\,k \neq 0 \\
    0                                         & \text{else}             \\
  \end{cases}
\end{align*}

Unfortunately, as the following lemma shows, it is not possible to use semimodules for aggregation over $\uaaN$-relations, because such semimodules, if they exist, cannot be bound preserving.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{Applying Semimodules to $\uaaK{\semN}$-Relations}
% \label{sec:semim-uaaks-relat}


\BG{DEL: As we will demonstrate, even though it may be possible to
define $\uaaN$-semimodules, such semimodules cannot be bound preserving.
% and, thus, would be useless for our purpose.
We show that it is
possible to define bound preserving operations $\mysmbNAU{\monoid}$ that combine $\uaaN$
elements with $\rangeDom$ elements and that this is sufficient for defining a
bound preserving aggregation semantics.}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{Lemma}\label{lem:bound-preserving-impossible}
$\smbpair_{\uaaK{\semN},\msum}$, if it is well-defined, is not bound preserving.
\end{Lemma}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{proof}[Proof Sketch]
  Assume that this semimodule exists and is bound preserving. We lead this assumption to a contradiction by deriving two different results for the expression $\ut{1}{1}{2} \smbNAU{\msum} \uv{0}{0}{0}$ using semimodule laws: (i) the obvious $\uv{0}{0}{0}$ and (ii) $\uv{-1}{0}{1} = \ut{1}{1}{2} \smbNAU{\msum} (\uv{-1}{-1}{-1} \addN \uv{1}{1}{1})$
  (full proof in \cite{techreport}).
  %show in \Cref{fig:semimodule-laws} under the assumption that the inputs are bounded .
\end{proof}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\iftechreport{Intuitively, an aggregate's bounds may be affected by order of operations, becoming weaker than strictly necessary.
While a stronger constraint is not efficiently enforceable, we can still require that the aggregate preserve bounds.
A naive non-semimodule definition of $\amysmbNAU$ might use point-wise application of
$\smbN{\monoid}$. However, this does not always preserve bounds. For instance, consider sum
aggregation ($\msum$) over
a $\uaaK{\semN}$-relation $\rangeRel(A)$ with a single tuple $\tuple{\uv{-3}{-2}{-1}}$
with annotation $\ut{0}{1}{1}$ and query $\aggnogb{sum(A)} (R)$. If
$\mysmbNAU{\msum}$ would be defined as point-wise application of
$\smbN{\msum}$, then the result of aggregation would be
$\uv{-3 \cdot 0}{-2 \cdot 1}{-1 \cdot 1} = \uv{0}{-2}{-1}$ which is not a
valid range-annotated value because $0 > -2$.
}
% The reason why point-wise application fails is that $\smbN{\msum}$
% does not preserve the order of the domain $\dataDomain$ based on which we
% defined range-annotated values.
% As we already saw in \Cref{sec:range-expr-eval},
% that multiplication over $\rangeDom$ cannot be defined pointwise to preserve
% bounds.
In spite of this negative result, not everything is lost. Observe that it not necessary for the operation that combines semiring elements (tuple annotations) with elements of the aggregation monoid to follow semimodule laws. After all, what we care about is that the operation is bound-preserving.
Below we define operations $\mysmbNAU{\monoid}$ that are not semimodules, but are bound-preserving.
To achieve bound-preservation we can rely on the bound-preserving expression semantics we have defined in~\Cref{sec:expression}.
For example,
% We show that it is
% possible to define bound preserving operations $\mysmbNAU{\monoid}$ that combine $\uaaN$
% elements with $\rangeDom$ elements and that this is sufficient for defining a
% bound preserving aggregation semantics.
since $\smbN{\msum}$ is multiplication, we can define
$\mysmbNAU{\msum}$ using multiplication for range-annotated values. % \revm{which we did already prove to be bound preserving}.
This approach of computing the bounds as the  minimum and maximum over all pair-wise combinations of value and tuple-annotation bounds also works for $\mmin$ and $\mmax$.
In~\cite{techreport} we prove that $\amysmbNAU$ is in fact bound preserving.
% The idea applied in
% the definition below is the same as uses in the definition of multiplication
% over range-annotated values: evaluate $\smbpair_{\semK,\monoid}$ over all
% combinations of values from the input and then return the minimum and maximum
% values over this set as bounds.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{Definition}\label{def:range-semimodules}
  Consider a monoid $\monoid \in \{\msum, \mmin, \mmax\}$. % such that $\smbN{\monoid}$ is well defined.
  Let $\uv{\lbMarker{m}}{m}{\ubMarker{m}}$ be a range-annotated value from $\rangeDom$ and $\ut{\lbMarker{k}}{k}{\ubMarker{k}} \in \uaaK{\semN}$.
  %Let triple  that  the value domain. Let triple $\semNX^3=(\lbMarker{x},x,\ubMarker{x})$ denote a tuple annotation value in \abbrAUDB.
We define $\ut{\lbMarker{k}}{k}{\ubMarker{k}} \amysmbNAU \uv{\lbMarker{m}}{m}{\ubMarker{m}} =$
%  We define $\amysmbNAU$ as shown below. % range aggregation monoid multiplication computation yields a triple as below.
  % \begin{flalign*}
  %     \ut{\lbMarker{k}}{k}{\ubMarker{k}} \amysmbNAU \uv{\lbMarker{m}}{m}{\ubMarker{m}} =
  % \end{flalign*}
%%%%%%%%%%%%%%%%%%%%
  \begin{align*}
		[& min(\lbMarker{k} \smbN{\monoid} \lbMarker{m},\lbMarker{k} \smbN{\monoid} \ubMarker{m},\ubMarker{k} \smbN{\monoid} \lbMarker{m},\ubMarker{k} \smbN{\monoid} \ubMarker{m}), \\
		& {k} \smbN{\monoid} {m}, \\
		& max(\lbMarker{k} \smbN{\monoid} \lbMarker{m},\lbMarker{k} \smbN{\monoid} \ubMarker{m},\ubMarker{k} \smbN{\monoid} \lbMarker{m},\ubMarker{k} \smbN{\monoid} \ubMarker{m})]
	\end{align*}

\end{Definition}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Note that, in general there is no guarantee that
% $\smbpair_{\uaaK{\semK},\monoid}$ according to \Cref{def:range-semimodules}
% preserves bounds. However,


% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{Lemma}\label{theo:uaa-semimodules-preserve-bounds}
% $\amysmbNAU$ is bound preserving for $\monoid \in \{\mmin, \mmax, \msum\}$. % we have that .
% \end{Lemma}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{proof}[Proof Sketch]
% We have to show for all $\monoid \in \{\mmin, \mmax, \msum\}$ that for any $\vec{k} = \ut{\lbMarker{k}}{\bgMarker{k}}{\ubMarker{k}} \in \uaaK{\semN}$ and $\vec{m} = \uv{\lbMarker{m}}{\bgMarker{m}}{\ubMarker{m}} \in \rangeDom$ we have that $\vec{k} \amysmbNAU \vec{m}$ bounds $k \smbN{\monoid} m$ for any $k$ bound by $\vec{k}$ and $m$ bound by $\vec{m}$. The claim is proven by substitution of definitions and case distinctions (are the annotation bounds $0$ or not and are one or both bounds of $\vec{m}$ negative). See~\cite{techreport} for the full proof.
% \end{proof}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Bound-Preserving Aggregation}
\label{sec:bound-pres-aggr}
We now define a bound preserving aggregation semantics based on the
$\amysmbNAU$ operations. % As mentioned above, the main
% challenge we have to overcome is to deal with the uncertainty of group
% memberships plus the resulting uncertainty in the number of groups and of which
% inputs contribute to a group's aggregation function result values.
% In general,
% the number of possible groups encoded by an input \abbrUAADB-relation may be
% very large.
% Thus, enumerating all concrete groups is not a viable option.  While
Since \abbrUAADBs can be used to encode an arbitrary number of groups as a single
tuple, we need to decide how to trade conciseness of the representation for
accuracy. Furthermore, we need to ensure that the aggregation result in the
\abbrBGW is encoded by the result. There are many possible strategies for how to
group possible aggregation results. In this paper, we limit the discussion to a default strategy  that we introduce next (see~\cite{techreport} for a general treatment). % we formalize grouping strategies and define a semantics for aggregation that preserves bounds for any such grouping semantics.
% We define our aggregation semantics in three steps: (i) we introduce our default grouping strategy that matches \abbrBG and possible input groups to output tuples (each output tuple will represent exactly one group in the  \abbrBGW and one or more possible groups);
Afterwards,  we demonstrate how to calculate group-by attribute and aggregation result ranges for output tuples.
% based on the assignment of input tuples to output tuples; (iii) we calculate the multiplicities and bounds for aggregation function results for each output tuple. % based on the grouping strategy.


  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\mypar{Grouping Strategy}
Our \textit{grouping strategy}
takes as input an n-ary $\uaaK{\semN}$-relation $\rangeRel$ and a list of group-by attributes $\gbAttrs$ and returns a pair $(\stratGrps, \stratPoss)$ where $\stratGrps(\gbAttrs, \rangeRel)$ is a set of output tuples --- one for every \abbrBG group (an input tuple's group-by values in the \abbrBGW), and
$\stratPoss$ assigns each input tuple to one output based on its \abbrBG group-by values.
Even if the \abbrBG annotation of an input tuple is $0$, we still use its \abbrBG values
  to assign it to an output tuple.
  Only tuples that are not possible (annotated with $\uaaZero{\semN} = \ut{0}{0}{0}$) are not considered.
  Since output tuples are identified by their \abbrBG group-by values, we will use these values to  identify elements from $\stratGrps$.
  % All possible groups of an input tuple are associated with the output that corresponds to the tuple's group-by values in the \abbrBGW.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \begin{Definition}% [Default Grouping Strategy]
    \label{def:default-grouping-strategy}
Consider a query $\query \defas \aggregation{\gbAttrs}{f(A)}(\rangeRel)$.
  Let $\rangeTup \in \rangeDom^n$. % such that $\rangeRel(\rangeTup) \neq \zeroOf{\uaaK{\semN}}$ and $\rangeTup' \in \rangeDom^n$ such that $\bgMarker{\rangeRel(\rangeTup')} \neq \zeroN$.
 The default grouping strategy $\gsdef \defas (\gsdefG,  \gsdefP)$ is defined as:
\begin{align*}
 \gsdefG(\gbAttrs, \rangeRel)                      & \defas  \{ t.\gbAttrs \mid \exists \rangeTup: \bgMarker{\rangeTup} = t \wedge \rangeRel(\rangeTup) \neq \uaaZero{\semN} \} &
  % \gsdefBG(\rangeTup')        & \defas \bgMarker{\rangeTup'.\gbAttrs}  &
  \gsdefP(\rangeTup)          & \defas \bgMarker{\rangeTup.\gbAttrs}
\end{align*}
\end{Definition}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Note that one range-annotated input tuple may belong to multiple groups since
% its group-by values may bound multiple \abbrBG groups.
For instance, consider
three tuples $\rangeTup_1 \defas \tuple{\uv{1}{2}{2}}$ and
$\rangeTup_2 \defas \tuple{\uv{2}{2}{4}}$ and $\rangeTup_3 \defas \tuple{\uv{2}{3}{4}}$ of a relation $\rangeRel(A)$.
Furthermore, assume that $\rangeRel(\rangeTup_1) = \ut{1}{1}{1}$, $\rangeRel(\rangeTup_2) = \ut{0}{0}{1}$, and
$\rangeRel(\rangeTup_3) = \ut{0}{0}{3}$.
Grouping on $A$,
the default strategy will generate  two output groups $\agroup_1$ for \abbrBG group $(2)$ and
$\agroup_2$ for \abbrBG group $(3)$.
% Tuple $\rangeTup_1$ is the only tuple that is present in the \abbrBGW. Function $\gsdefBG$ assigns $\rangeTup_1$ to $\agroup_1$.
Based on their \abbrBG group-by values, $\gsdefP$ assigns $\rangeTup_1$ and $\rangeTup_2$ to $\agroup_1$ and $\rangeTup_3$ to $\agroup_2$.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\mypar{Aggregation Semantics}
%
We now introduce an aggregation semantics based on this grouping strategy.  For
simplicity we define aggregation without group-by as a special case of
aggregation with group-by (the only difference is how tuple annotations are
handled). We first define how to construct a result tuple $\aout$ for each
output group $\asgrp$ returned by the grouping strategy and then present how to
calculate tuple annotations. The construction of an output tuple is divided into
two steps: (i) determine range annotations for the group-by attributes and (ii)
determine range annotations for the aggregation function result attributes.  To
ensure that all possible groups that an input tuple $\rangeTup$ with
$\gsdefP(\rangeTup) = \asgrp$ belongs to are contained in $\aout.\gbAttrs$ we
have to merge the group-by attribute bounds of all of these tuples. Furthermore,
we use the unique \abbrBG group-by values common to all input tuples assigned to $\aout$ (i.e., $\bgMarker{\aout.\gbAttrs} = \asgrp$) as the output's \abbrBG group-by value.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{Definition}% [Range-bounded Groups]
  \label{def:range-bounded-groups}
Consider a result group $\asgrp \in \gsdefG(\gbAttrs, \rangeRel)$ for an aggregation with group-by attributes $\gbAttrs$ over a $\uaaK{\semN}$-relation $\rangeRel$. The bounds for the group-by attributes values of $\aout$ are defined as shown below. % Let $\agroup$ be the unique element from the set $\{ \bgMarker{\rangeTup.\gbAttrs} \mid \bgMarker{\rangeRel(\rangeTup)} \neq 0 \wedge \stratPoss(\rangeTup) = \aout \}$.
For all $a \in \gbAttrs$ we define:\\[-5mm]
%%%%%%%%%%%%%%%%%%%%
\begin{align*}
\lbMarker{\aout.a} &= \min_{\rangeTup: \stratPoss(\rangeTup) = \asgrp} \lbMarker{\rangeTup.a} &
\bgMarker{\aout.a} &= \agroup.a &
\ubMarker{\aout.a} &= \max_{\rangeTup: \stratPoss(\rangeTup) = \asgrp} \ubMarker{\rangeTup.a}
\end{align*}
\end{Definition}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Note that in the definition above, $\min$ and $\max$ are the minimum and maximum
wrt. to the order over the data domain $\dataDomain$ which we used to define
range-annotated values.  Reconsider the three example tuples and two result groups from above.
The group-by range annotation for output tuple $\outof{\agroup_1}$ is
$\uv{\min(1,2)}{2}{\max(2,4)} = \uv{1}{2}{4}$. Observe that $\uv{1}{2}{4}$ bounds
every group $\rangeTup_1$ and $\rangeTup_2$ may belong to in some possible world.
To calculate bounds on the result of an aggregation function for one group, we have to reason about the minimum and maximum possible aggregation function result based on the bounds of aggregation function input values, their associated row annotations, and their possible and guaranteed group memberships. % Even when an aggregation function input value is certain, which group the tuple belongs may be uncertain.
To calculate a conservative lower bound of the aggregation function result for an output tuple $\aout$, we use $\amysmbNAU$ to pair the aggregation function value of each tuple $\rangeTup$ for which $\stratPoss(\rangeTup) = \asgrp$ holds with the tuple's annotation and then extract the lower bound from the resulting range-annotated value.
The group membership of a contributing tuple is uncertain if either its group-by values are uncertain or if it need not exist in all possible worlds (its certain multiplicity is $0$).
We thus take the minimum of the neutral element of the aggregation monoid and the result of $\amysmbNAU$ for such tuples. We introduce an \emph{uncertain group} predicate $\uncertg{\gbAttrs}{\rangeRel}{\rangeTup}$ for this purpose:\\[-5mm]
% that is defined as shown below.
%
\begin{align*}
  \uncertg{\gbAttrs}{\rangeRel}{\rangeTup} \defas (\exists a \in \gbAttrs: \lbMarker{\rangeTup.a} \neq \ubMarker{\rangeTup.a}) \vee \lbMarker{\rangeRel(\rangeTup)} = 0
\end{align*}
%
We then sum up the resulting values in the aggregation monoid. Note that here summation is addition in $\monoid$. % The result for each tuple belong to the group $\tgrouping(\agroup)$.
The upper bound calculation is analogous (using the upper bound and maximum instead). The \abbrBG result is calculated using standard $\semN$-relational semantics. We use $\rangeTup \toverlaps \rangeTup'$ to denote that the range annotations of tuples $\rangeTup$ and $\rangeTup'$ with the same schema $(A_1, \ldots, A_n)$ overlap on each attribute $A_i$, i.e.,\\[-4mm]
%
\begin{align*}
\rangeTup \toverlaps \rangeTup' \defas \bigwedge_{i \in \{1, \ldots, n\}} [ \lbMarker{\rangeTup.A_i}, \ubMarker{\rangeTup.A_i} ] \cap  [ \lbMarker{\rangeTup'.A_i}, \ubMarker{\rangeTup'.A_i} ] \neq \emptyset
\end{align*}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{Definition}% [Aggregation Function Result Bounds]
  \label{def:agg-function-bounds}
  Consider input $\rangeRel$, set of group-by
  attributes $\gbAttrs$, an output $\asgrp \in \gsdefG(\gbAttrs, \rangeRel)$,
  and aggregation function $f(A)$ with monoid $\monoid$.
  We use $\tgrouping(\asgrp)$ to denote the set of inputs with group-by
  attribute bounds overlaping $\aout.\gbAttrs$, i.e., belonging to a
  group represented by $\aout$:\\[-5mm]
  %%%%%%%%%%%%%%%%%%%%
  \begin{align*}
    \tgrouping(\asgrp) \defas \{ \rangeTup \mid \rangeRel(\rangeTup) \neq \uaaZero{\semN} \wedge \rangeTup.\gbAttrs \toverlaps \aout.\gbAttrs\}
  \end{align*}
  %%%%%%%%%%%%%%%%%%%%
  The aggregation function result bounds for tuple $\aout$ are defined as: \\[-3mm]
  %%%%%%%%%%%%%%%%%%%%
  \begin{align*}
    \lbMarker{\aout.f(A)} &= \sum_{\rangeTup \in \tgrouping(\asgrp)} \lbagg{\rangeTup}
  &\ubMarker{\aout.f(A)} &= \sum_{\rangeTup \in \tgrouping(\asgrp)} \ubagg{\rangeTup}
  \end{align*}\\[-6mm]
  \begin{align*}
     \bgMarker{\aout.f(A)} &= \sum_{\rangeTup \in \tgrouping(\asgrp)} \bgMarker{(\rangeRel(\rangeTup) \amysmbNAU \rangeTup.A)}
  \end{align*}\\[-6mm]
  %%%%%%%%%%%%%%%%%%%%
  \begin{align*}
  \lbagg{\rangeTup}     &= \begin{cases}
                            min(\amzero,\lbMarker{(\rangeRel(\rangeTup) \amysmbNAU \rangeTup.A)}) &\mathtext{if }\uncertg{\gbAttrs}{\rangeRel}{\rangeTup} \\
                            \lbMarker{(\rangeRel(\rangeTup) \amysmbNAU \rangeTup.A)} &\mathtext{otherwise}\\
                          \end{cases}\\
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \ubagg{\rangeTup}     &= \begin{cases}
                            max(\amzero,\ubMarker{(\rangeRel(\rangeTup) \amysmbNAU \rangeTup.A)}) &\mathtext{if }\uncertg{\gbAttrs}{\rangeRel}{\rangeTup} \\
                            \ubMarker{(\rangeRel(\rangeTup) \amysmbNAU \rangeTup.A)}&\mathtext{otherwise}\\
                          \end{cases}
  % \lbMarker{\aout(\agroup).f(A)} &= \sum_{\rangeTup.\gbAttrs \tmatch \aout(\agroup).\gbAttrs}min(\amzero,\lbMarker{(\rangeRel(\rangeTup) \smbpair_{\uaaK{\semK}} \rangeTup.A)}) \\
  %  \bgMarker{\aout(\agroup).f(A)} &= \sum_{\rangeTup.\gbAttrs \tmatch \aout(\agroup).\gbAttrs}\bgMarker{(\rangeRel(\rangeTup) \smbpair_{\uaaK{\semK}} \rangeTup.A)} \\
  %  \ubMarker{\aout(\agroup).f(A)} &= \sum_{\rangeTup.\gbAttrs \tmatch \aout(\agroup).\gbAttrs}max(\amzero,\ubMarker{(\rangeRel(\rangeTup) \smbpair_{\uaaK{\semK}} \rangeTup.A)}) \\
\end{align*}
\end{Definition}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{Example}
  For instance, consider calculating the sum of $A$ grouping on $B$ for a relation $R(A,B)$, which consists of two tuples $\rangeTup_1 \defas \tuple{\uv{3}{5}{10},\uv{3}{3}{3}}$ and $\rangeTup_2 \defas \tuple{\uv{-4}{-3}{-3},\uv{2}{3}{4}}$ that are both annotated with \ut{1}{2}{2} (appear certainly once and may appear twice). Consider calculating the aggregation function result bounds for the result tuple $\aout$ for the output group $\asgrp \defas \tuple{3}$. The lower bound $\sum_{\rangeTup \in \tgrouping(\asgrp)} \lbagg{\rangeTup}$ on {\upshape \lstinline!sum(A)!} is calculated (\Cref{def:range-semimodules}) as:
  \begin{align*}
    % &\sum_{\rangeTup \in \tgrouping(\asgrp)} \lbagg{\rangeTup}\\
    = &\lbMarker{\left(\ut{1}{2}{2} \cdot \uv{3}{5}{10}  \right)} + min(0, \lbMarker{\left(\ut{1}{2}{2} \cdot \uv{-4}{-3}{-3}\right)})\\
    = &\lbMarker{\uv{3}{10}{20}} + min(0, \lbMarker{\uv{-8}{-6}{-3}})
    =3 + min(0,-8) = -5
  \end{align*}
The aggregation result is guaranteed to be greater than or equal to $-5$ since $\rangeTup_1$ certainly belongs to $\asgrp$   (no minimum operation), because its group-by attribute value $\uv{3}{3}{3}$ is certain and the tuple certainly exists ($\lbMarker{\ut{1}{2}{1}} > 0$). This tuple contributes $3$ to the sum and $\rangeTup_2$ contributions at least $-8$. While it is possible that $\rangeTup_2$ does not belong to $\asgrp$ this can only increase the final result ($3 + 0 > 3 + -8$).
\end{Example}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% As shown in the example above, we can tighten the bounds on aggregation function result if we take into account that some tuples certainly belong to a particular group (their group-by values are certain). This can be realized by only conditionally applying the minimum (maximum) operation in the calculation of the bounds when a tuple has uncertain group-by values.
% \BG{We apply this in our implementation? This should be cheap?}
% \BG{Should define a predicate that checks whether tuple's values are certain. Then this could be included into the definition without causing to much complexity increase.}
We still need to calculate the multiplicity annotation for each result tuple. For aggregation without group-by, there is always exactly one result tuple.
In this case there exists a single possible \abbrBG output group (the empty tuple $\tuple{}$ ) and all input tuples are assigned to it through $\gsdefP$. Let $\rangeTup_{\tuple{}}$ denote this single output tuple.
Recalling that all remaining tuples have multiplicity $\zeroN$, we define:  % $\ggrouping(\emptyset, \rangeRel)$ will consist of a single group $()$ containing all input tuples.
  \begin{align*}
    \lbMarker{\aggregation{}{f(A)}(\rangeRel)(\rangeTup)}
    =     \bgMarker{\aggregation{}{f(A)}(\rangeRel)(\rangeTup)}
    =     \ubMarker{\aggregation{}{f(A)}(\rangeRel)(\rangeTup)}
    \defas \begin{cases}
      \oneN &\text{if}\,\,\, \rangeTup = \rangeTup_{\tuple{}}\\
      \zeroN & \text{otherwise}
    \end{cases}
  \end{align*}

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{Definition}[Aggregation Without Group-By]\label{def:aggr-op-semantics-wo-gb}
%   Consider a query $\query \defas \aggregation{}{f(A)}(\rangeRel)$. Let
% $\gsdef(\emptyset,\rangeRel) = (\gsdefG, \gsdefP)$,
%   and $\rangeTup$  be a range-annotated tuple with the same schema as $\query$ and $\asgrp$ denote the single output group in $\gsdefG$. Then
%   \begin{align*}
%     \lbMarker{\aggregation{}{f(A)}(\rangeRel)(\rangeTup)}
%     =     \bgMarker{\aggregation{}{f(A)}(\rangeRel)(\rangeTup)}
%     =     \ubMarker{\aggregation{}{f(A)}(\rangeRel)(\rangeTup)}
%     \defas \begin{cases}
%       \oneN &\text{if}\,\,\, \rangeTup = \aout\\
%       \zeroN & \text{otherwise}
%     \end{cases}
%   \end{align*}
% % We define a predicate $\rangeTup \equiv \rangeTup'$ that evaluates to true iff $\rangeTup=\rangeTup'$ and both $\rangeTup$ and $\rangeTup'$ are certain and a predicate $\rangeTup \matches \rangeTup'$ that evaluates to true iff $\forall i \in \{1, \ldots, n\}: \lbMarker{\rangeTup.a_i} \ordK
% \end{Definition}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In order to calculate the upper bound on the possible multiplicity for a result tuple of a group-by aggregation, we have to determine the maximum number of distinct groups this output tuple could correspond to.
We compute the bound for an output $\aout$ based on $\ggrouping$ making the worst-case assumption that
(i) each input tuple $\rangeTup$ with $\gsdefP(\rangeTup) = \asgrp$ has the maximal multiplicity possible ($\ubMarker{\rangeRel(\rangeTup)}$);
(ii) each tuple $\tup$ encoded by $\rangeTup$ is in a separate group; and
(iii) groups produced from two inputs $\rangeTup$ and $\rangeTup'$ do not overlap.
We can improve this bound by partitioning the input into two sets: tuples with uncertain group-by values and tuples with certain group membership.
When calculating the maximum number of groups for an output $\aout$, the set of input tuples with certain group-by values that fall into the group-by bounds of $\aout$ only contribute the number of distinct \abbrBG group-by values from this set to the bound.
% For the latter we can compute the maximum number of groups for an output $\aout$ by simplying counting the number of groups using \abbrBG values for each input tuple that overlaps with the group-by bounds of $\aout$.
%
For the first set we still apply the worst-case assumption.
To determine the lower bound on the certain annotation of a tuple we have to reason about which input tuples certainly belong to a group. These are inputs whose group-by attributes are certain. For such tuples we sum up their tuple annotation lower bounds.
We then need to derive the annotation of a result tuple from relevant input tuple annotations. \cite{amsterdamer2011provenance} extended semirings with a duplicate elimination operator $\duprem_\semN$ for this purpose which is
defined as $\duprem_\semN(k) = 0$ if $k = 0$ and $\duprem_{\semN}(k) = 1$ otherwise.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{Definition}% [Aggregation With Group-By]
  \label{def:aggr-op-semantics-gb}
 Let $\query \defas \aggregation{\gbAttrs}{f(A)}(\rangeRel)$ and $\gsdef(\rangeRel,\gbAttrs) = (\gsdefG, \gsdefP)$.
% We define a predicate $\rangeTup \equiv \rangeTup'$ that evaluates to true iff $\rangeTup=\rangeTup'$ and both $\rangeTup$ and $\rangeTup'$ are certain and a predicate $\rangeTup \matches \rangeTup'$ that evaluates to true iff $\forall i \in \{1, \ldots, n\}: \lbMarker{\rangeTup.a_i} \ordK \lbMarker{\rangeTup'.a_i} \ordK \ubMarker{\rangeTup.a_i} \vee \lbMarker{\rangeTup.a_1} \ordK \ubMarker{\rangeTup'.a_i} \ordK \ubMarker{\rangeTup.a_i}$. Using these predicates we define set difference as shown below.%
Consider a tuple $\rangeTup$ such that $\exists \asgrp \in \gsdefG$ with $\rangeTup = \aout$. Then,\\[-4mm]
%
\begin{align*}
	\lbMarker{\aggregation{\gbAttrs}{f(A)}(\rangeRel)(\rangeTup)} &\defas  \duprem_{\semN}\left(\sum_{\rangeTup': \gsdefP(\rangeTup') = \asgrp \wedge \neg\, \uncertg{\gbAttrs}{\rangeRel}{\rangeTup'}}\lbMarker{\rangeRel(\rangeTup')}\right) \\
%%%%%%%%%%%%%%%%%%%%
  \bgMarker{\aggregation{\gbAttrs}{f(A)}(\rangeRel)(\rangeTup)} &\defas       \duprem_{\semN}\left(\sum_{\rangeTup': \gsdefP(\rangeTup') = \asgrp} \bgMarker{\rangeRel(\rangeTup')}\right)\\
%%%%%%%%%%%%%%%%%%%%
     \ubMarker{\aggregation{\gbAttrs}{f(A)}(\rangeRel)(\rangeTup)} &\defas
\sum_{\rangeTup': \gsdefP(\rangeTup') = \asgrp} \ubMarker{\rangeRel(\rangeTup')}
%%%%%%%%%%%%%%%%%%%%
\end{align*}
For any tuple $\rangeTup$ such that $\neg \exists \asgrp \in \gsdefG$ with $\rangeTup = \aout$, we define
\[
  \lbMarker{\aggregation{\gbAttrs}{f(A)}(\rangeRel)(\rangeTup)} =
  \bgMarker{\aggregation{\gbAttrs}{f(A)}(\rangeRel)(\rangeTup)} =
  \ubMarker{\aggregation{\gbAttrs}{f(A)}(\rangeRel)(\rangeTup)}
  = 0
\]
\end{Definition}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\begin{figure}[t]
  \centering

    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \begin{subtable}{\linewidth}
  \centering
  \begin{tabular}{ c|c|cc}
    \textbf{street}  & \textbf{number}          & \thead{\#inhab} & \underline{$\uaaK{\semN}$} \\
    \cline{1-3}
      \cMarker{Canal}    & $\uv{165}{165}{165}$     & $\uv{1}{1}{1}$  & (1,1,2)                    \\
%       \cline{1-3}
    \uMarker{Canal}  & $\uv{154}{153}{156}$     & $\uv{1}{2}{2}$  & (1,1,1)                    \\
%       \cline{1-3}
    \cMarker{State}  & $\uv{623}{623}{629}$     & $\uv{2}{2}{2}$  & (2,2,3)                    \\
    \cMarker{Monroe} & $\uv{3574}{3550}{3585}$  & $\uv{2}{3}{4}$  & (0,0,1)                    \\
%       \cline{1-3}
  \end{tabular}\\[-1mm]
  \caption{Input relation address}
        \label{fig:AU-agg-example-input}
  \end{subtable}\\[-1mm]
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%   \begin{subtable}{\linewidth}
%   \centering
% \begin{lstlisting}
% SELECT sum(#inhab) AS pop FROM address;
% \end{lstlisting}
%   \begin{tabular}{ cc}
% %       \cline{1-2}
%  \textbf{pop}   & \underline{$\uaaK{\semN}$} \\
% \cline{1-1}
%  $\uv{6}{7}{14}$ & (1,1,1)                    \\
% %       \cline{1-2}
%   \end{tabular}
%   \caption{Aggregation without Group-by}
%     \label{fig:AU-agg-example-no-GB}
%   \end{subtable}
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \begin{subtable}{\linewidth}
  \centering
    \begin{minipage}{0.49\linewidth}
\begin{lstlisting}
SELECT street,
       count(*) AS cnt
FROM address
GROUP BY street;
\end{lstlisting}
    \end{minipage}
    \begin{minipage}{0.49\linewidth}
      \centering
  \begin{tabular}{ c|cc}
      % \cline{1-2}
    \textbf{street}  & \textbf{cnt}   & \underline{$\uaaK{\semN}$} \\
    \cline{1-2}
    \uMarker{Canal}  & $\uv{1}{2}{3}$ & (1,1,2)                    \\
    \cMarker{State}  & $\uv{2}{2}{4}$ & (1,1,1)                    \\
    \cMarker{Monroe} & $\uv{1}{1}{2}$ & (0,0,1)                    \\
      % \cline{1-2}
  \end{tabular}
  \end{minipage}\\[-3mm]
    \caption{Aggregation with Group-by}
    \label{fig:AU-agg-example-GB}
  \end{subtable}\\[-3mm]
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\caption{Aggregation over \abbrUAADBs}
\label{fig:AU-aggregation}
\trimfigurespacing
\end{figure}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{Optimizing Bounds}
% \label{sec:optimizing-bounds}

% The bounds provided by the  general aggregation semantics introduced above can be improved if we take the semantics of the aggregation function into account. In the following we provide better bounds for \aggsum, and \BG{What else?}

% unless the aggregation domain is extended to be symbolic expressions over semiring elements paired with monoid values combined by an abstract addition operation.


% hand demonstrated how to  keep the size of a query result polynomial in the input size of the query by representing the result of aggregation function results as symbolic expressions that pair semiring values with values of the aggregation domain. For instance, without going too much into technical detail, in semiring $\semNX$ the result of a sum aggregation may be $3 \otimes x_1 +_{sum} 2 \otimes x_2$ which intuitively means that the final result of the sum of value $3$ subject to variable $x_1$ and value $2$ subject to variable $x_2$.


% \BG{Is a a more general semantics we can define and then refine for tighter bounds? What about min/max?}

% \BG{Fix notation in the rewrites. Explain notation that is new (attribute names and such)}
% \BG{Define aggregation as an operator, not just aggregation function results}
% %\subsubsection{Row bounds}
% %

% We start with a more general form of the aggregation rule by using polynomial representations. In the real use cases we consider the limitation on the polynomial such that the polynomial can be evaluated into a concrete value.\SF{Do we?} In this case the definition of upper and lower bounds are clear.

% \BG{Not sure whether we need to reiterate this here, but keep it for now:}
% Recall that $\rangeTup[A]$ outputs projection of tuple $\rangeTup$ on a set of attributes $A$.

% \BG{Probably use $f(a)$ instead of $f$ to indicate what attribute we are aggregating over.}

% \BG{We still have to define the aggregation function result for a set of tuples to be able to restrict $\rangeTup$ to tuples that should be in the result instead of just tuples that have the right GB values.}

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{Definition}[Aggregation Operator]\label{def:aggr-op-semantics}
% Let $\rangeTup$ and $\rangeTup'$ be range-annotated tuples where $\rangeTup$ has the same arity as $\aggregation{G}{f}(\rangeRel)$ and $\rangeTup'$ has the same arity as $\rangeRel$. Let $G$ be a set of group by attributes and $f$ be the aggregation function.  We define aggregation as shown below.
%    %We define a predicate $\rangeTup \equiv \rangeTup'$ that evaluates to true iff $\rangeTup=\rangeTup'$ and both $\rangeTup$ and $\rangeTup'$ are certain and a predicate $\rangeTup \matches \rangeTup'$ that evaluates to true iff $\forall i \in \{1, \ldots, n\}: \lbMarker{\rangeTup.a_i} \ordK \lbMarker{\rangeTup'.a_i} \ordK \ubMarker{\rangeTup.a_i} \vee \lbMarker{\rangeTup.a_1} \ordK \ubMarker{\rangeTup'.a_i} \ordK \ubMarker{\rangeTup.a_i}$. Using these predicates we define set difference as shown below.%
%    \begin{align*}
% 	\lbMarker{\aggregation{G}{f}(\rangeRel)(\rangeTup)} &\defas
% 	\begin{cases}
% 	1_k & \text{if } \exists_{\rangeTup'}:\bgMarker{\rangeTup[G]}=\bgMarker{\rangeTup'[G]} \\
% 		& \text{ and } \forall_{a \in G}:\lbMarker{\rangeTup'.a}=\ubMarker{\rangeTup'.a} \\
% 		& \text{ and } \lbMarker{\combine(\rangeRel)(\rangeTup)} > 0_k \\
% 	0_k & \text{else}
% 	\end{cases}
% 	\end{align*}
% 	\begin{align*}
% 	\bgMarker{\aggregation{g}{f}(\rangeRel)(\rangeTup)} &\defas \sum_{\bgMarker{\rangeTup[g]} = \bgMarker{\rangeTup'[g]}}\bgMarker{\combine(\rangeRel)(\rangeTup')}
% 	\end{align*}
% 	\begin{align*}
% 	\ubMarker{\aggregation{g}{f}(\rangeRel)(\rangeTup)} &\defas \sum_{\rangeTup[g] \matches \rangeTup'[g]}\ubMarker{\combine(\rangeRel)(\rangeTup')}
% 	\end{align*}
% \end{Definition}

% \begin{Definition}[Aggregation group by attributes]\label{def:aggr-grpby-attr-semantics}
% 	With similar notations, we define aggregation group by attribute bounds as shown below.
% 	\begin{align*}
% 		\forall_{a \in g}:\lbMarker{\aggregation{g}{f}(\rangeRel)(\rangeTup).a} &\defas \minOf{\rangeTup[G] \matches \rangeTup'[G]}\combine(\rangeRel)(\lbMarker{\rangeTup'.a}) \\
% 		\forall_{a \in g}:\ubMarker{\aggregation{g}{f}(\rangeRel)(\rangeTup).a} &\defas \maxOf{\rangeTup[G] \matches \rangeTup'[G]}\combine(\rangeRel)(\ubMarker{\rangeTup'.a})
% 	\end{align*}
% \end{Definition}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{Definition}[General aggregation result attributes]\label{def:aggr-gen-attr-semantics}
% 	Define operator $\{k\}^{+}$ and $\{k\}^{-}$ over value $k$ s.t.
% 	\begin{align*}
% 		\{k\}^{+} =
% 	\begin{cases}
% 	k & \text{if } k \text{ contributes to } \ubMarker{f} \\
% 	0_k & \text{else}
% 	\end{cases}
% 	\end{align*}
% 	\begin{align*}
% 		\{k\}^{-} =
% 	\begin{cases}
% 	k & \text{if } k \text{ contributes to } \lbMarker{f} \text{ but not } \ubMarker{f} \\
% 	0_k & \text{else}
% 	\end{cases}
% 	\end{align*}
% 	Use $a_f$ to denote the attribute used by function $f$. We define general aggregation result attribute bounds as shown below.
% 	\begin{align*}
% 		& \aggregation{g}{f}(\rangeRel)(\rangeTup). \lbMarker{f} \defas \\ & \sum_{\rangeTup'[g] \equiv \rangeTup[g]}\{\lbMarker{\rangeRel(\rangeTup')}*\rangeRel(\rangeTup').\lbMarker{a_f}\}^+ \oplus \sum_{\rangeTup'[g] \matches \rangeTup[g]} \{\ubMarker{\rangeRel(\rangeTup')}*\rangeRel(\rangeTup').\lbMarker{a_f}\}^- \\
% 		& \aggregation{g}{f}(\rangeRel)(\rangeTup). \bgMarker{f} \defas \\ & \sum_{\bgMarker{\rangeTup'[g]} = \bgMarker{\rangeTup[g]}}\bgMarker{\rangeRel(\rangeTup')}*\rangeRel(\rangeTup').\bgMarker{a_f} \\
% 		& \aggregation{g}{f}(\rangeRel)(\rangeTup). \ubMarker{f} = \\ & \sum_{\rangeTup'[g] \matches \rangeTup[g]}\{\ubMarker{\rangeRel(\rangeTup')}*\rangeRel(\rangeTup').\ubMarker{a_f}\}^+ \oplus \sum_{\rangeTup'[g] \equiv \rangeTup[g]} \{\lbMarker{\rangeRel(\rangeTup')}*\rangeRel(\rangeTup').\ubMarker{a_f}\}^-
% 	\end{align*}

% \end{Definition}


% \begin{Definition}[Sum aggregation result attributes]\label{def:sum-aggr-attr-semantics}
% 	Define operator $\{k\}^{+}$ and $\{k\}^{-}$ over value $k \in \semK$ s.t.
% 	\begin{align*}
% 		\{k\}^{+} =
% 	\begin{cases}
% 	k & \text{if } k > 0_k \\
% 	0_k & \text{else}
% 	\end{cases}
% 	\end{align*}
% 	\begin{align*}
% 		\{k\}^{-} =
% 	\begin{cases}
% 	k & \text{if } k < 0_k \\
% 	0_k & \text{else}
% 	\end{cases}
% 	\end{align*}
% 	We define sum aggregation result attribute bounds as shown below.
% 	\begin{align*}
% 		& \aggregation{g}{sum(a)}(\rangeRel)(\rangeTup). \lbMarker{sum(a)} \defas \\ & \sum_{\rangeTup'[g] \equiv \rangeTup[g]}\{\lbMarker{\rangeRel(\rangeTup')}*\rangeRel(\rangeTup').\lbMarker{a}\}^+ + \sum_{\rangeTup'[g] \matches \rangeTup[g]} \{\ubMarker{\rangeRel(\rangeTup')}*\rangeRel(\rangeTup').\lbMarker{a}\}^- \\
% 		& \aggregation{g}{sum(a)}(\rangeRel)(\rangeTup). \bgMarker{sum(a)} \defas \\ & \sum_{\bgMarker{\rangeTup'[g]} = \bgMarker{\rangeTup[g]}}\bgMarker{\rangeRel(\rangeTup')}*\rangeRel(\rangeTup').\bgMarker{a} \\
% 		& \aggregation{g}{sum(a)}(\rangeRel)(\rangeTup). \ubMarker{sum(a)} = \\ & \sum_{\rangeTup'[g] \matches \rangeTup[g]}\{\ubMarker{\rangeRel(\rangeTup')}*\rangeRel(\rangeTup').\ubMarker{a}\}^+ +\sum_{\rangeTup'[g] \equiv \rangeTup[g]} \{\lbMarker{\rangeRel(\rangeTup')}*\rangeRel(\rangeTup').\ubMarker{a}\}^-
% 	\end{align*}

% \end{Definition}

% \begin{Definition}[Count aggregation result attributes]\label{def:Count-aggr-attr-semantics}
% 	For count function, all values may contribute to both upper and lower bounds and all attribute values is assigned to $1_k$. The semantics can be simplified. We define count aggregation result attribute bounds as shown below.
% 	\begin{align*}
% 		& \aggregation{g}{count(a)}(\rangeRel)(\rangeTup). \lbMarker{count(a)} \defas \sum_{\rangeTup'[g] \equiv \rangeTup[g]}\lbMarker{\rangeRel(\rangeTup')} \\
% 		& \aggregation{g}{count(a)}(\rangeRel)(\rangeTup). \bgMarker{count(a)} \defas \sum_{\bgMarker{\rangeTup'[g]} = \bgMarker{\rangeTup[g]}}\bgMarker{\rangeRel(\rangeTup')} \\
% 		& \aggregation{g}{count(a)}(\rangeRel)(\rangeTup). \ubMarker{count(a)} \defas \sum_{\rangeTup'[g] \matches \rangeTup[g]}\ubMarker{\rangeRel(\rangeTup')}
% 	\end{align*}

% \end{Definition}

% \begin{Definition}[Min/Max aggregation result attributes]\label{def:MinMax-aggr-attr-semantics}
% 	For min/max function, all values may contribute to both upper and lower bounds, so the semantics can be simplified. We define Min/Max aggregation result attribute bounds as shown below.
% 	\begin{align*}
% 		& \aggregation{g}{min(a)}(\rangeRel)(\rangeTup). \lbMarker{min(a)} \defas \min_{\rangeTup'[g] \matches \rangeTup[g]}\lbMarker{\rangeRel(\rangeTup')} \\
% 		& \aggregation{g}{min(a)}(\rangeRel)(\rangeTup). \bgMarker{min(a)} \defas \min_{\bgMarker{\rangeTup'[g]} = \bgMarker{\rangeTup[g]}}\bgMarker{\rangeRel(\rangeTup')} \\
% 		& \aggregation{g}{min(a)}(\rangeRel)(\rangeTup). \ubMarker{max(a)} \defas \min_{\rangeTup'[g] \matches \rangeTup[g]}\ubMarker{\rangeRel(\rangeTup')}
% 	\end{align*}
% 	\begin{align*}
% 		& \aggregation{g}{max(a)}(\rangeRel)(\rangeTup). \lbMarker{max(a)} \defas \max_{\rangeTup'[g] \matches \rangeTup[g]}\lbMarker{\rangeRel(\rangeTup')} \\
% 		& \aggregation{g}{max(a)}(\rangeRel)(\rangeTup). \bgMarker{max(a)} \defas \max_{\bgMarker{\rangeTup'[g]} = \bgMarker{\rangeTup[g]}}\bgMarker{\rangeRel(\rangeTup')} \\
% 		& \aggregation{g}{max(a)}(\rangeRel)(\rangeTup). \ubMarker{max(a)} \defas \max_{\rangeTup'[g] \matches \rangeTup[g]}\ubMarker{\rangeRel(\rangeTup')}
% 	\end{align*}
% \end{Definition}



% %\begin{enumerate}
% %%\item selection
% %%\[\lbMarker{[\selection_\theta(R)](t)}=\lbMarker{R(t)} \otimes \lbMarker{(\theta(t))} \]
% %%\[\ubMarker{[\selection_\theta(R)](t)}=\ubMarker{R(t)} \otimes \ubMarker{(\theta(t))} \]
% %%
% %%\item join
% %%\[ \lbMarker{[R_1 \join R_2](t)} = \lbMarker{R_1(t)} \otimes \lbMarker{R_2(t)} \]
% %%\[ \ubMarker{[R_1 \join R_2](t)} = \ubMarker{R_1(t)} \otimes \ubMarker{R_2(t)} \]
% %%
% %%\item Union
% %%\[ \lbMarker{[R_1 \union R_2](t)} =
% %%	\lbMarker{R_1(t)} \oplus  \lbMarker{R_2(t)}\]
% %%\[ \ubMarker{[R_1 \union R_2](t)} = \ubMarker{R_1(t)} \oplus \ubMarker{R_2(t)} \]
% %%
% %%\item Projection
% %%\[ \lbMarker{[\projection_{U}(R)](t)} = \sum_{t=t'[U]}\lbMarker{R(t')} \]
% %%\[ \ubMarker{[\projection_{U}(R)](t)} = \sum_{t=t'[U]}\ubMarker{R(t')} \]
% %%
% %%\item Set difference
% %%\[ \lbMarker{[R_1 - R_2](t)} = \lbMarker{R_1(t)} \ominus \sum_{R_1(t) \matches R_2(t')} \ubMarker{R_2(t')} \]
% %%\[ \ubMarker{[R_1 - R_2](t)} = \ubMarker{R_1(t)} \ominus \sum_{R_1(t) \equiv R_2(t')} \lbMarker{R_2(t')} \]
% %
% %%\subsubsection{Attribute bound}
% %%\begin{enumerate}
% %
% %%\item Union
% %%\[ \forall_{a_i \in U } : [R_1 \union R_2](t).\lbMarker{a_i} = \min(R_1(t).\lbMarker{a_i},R_2(t).\lbMarker{a_i}) \]
% %%\[ \forall_{a_i \in U } : [R_1 \union R_2](t).\ubMarker{a_i} = \max(R_1(t).\ubMarker{a_i},R_2(t).\ubMarker{a_i}) \]
% %%
% %%\item Projection
% %%\[ \forall_{a_i \in U } : [\projection_{U}(R)](t).\lbMarker{a_i} = \min_{t=t'[U]} R(t').\lbMarker{a_i} \]
% %%\[ \forall_{a_i \in U } : [\projection_{U}(R)](t).\ubMarker{a_i} = \max_{t=t'[U]} R(t').\ubMarker{a_i} \]
% %
% %
% %
% %\item Count Aggregation without group by
% %\[ [ \aggregation{}{count(A)}(R) ](t).\lbMarker{count(A)} = \sum_{t' \in R}\lbMarker{R(t')} \]
% %\[ [ \aggregation{}{count(A)}(R) ](t).\ubMarker{count(A)} = \sum_{t' \in R}\ubMarker{R(t')} \]
% %
% %\item Count Aggregation with group by
% %\[ \forall_{a_i \in g } : [ \aggregation{g}{count(A)}(R) ](t).\lbMarker{a_i} = \min_{[\projection_{g}(R)](t[g]) \matches R(t')[g]} R(t').\lbMarker{a_i} \]
% %\[ \forall_{a_i \in g } : [ \aggregation{g}{count(A)}(R) ](t).\ubMarker{a_i} = \max_{[\projection_{g}(R)](t[g]) \matches R(t')[g]} R(t').\ubMarker{a_i} \]
% %
% %\[ [ \aggregation{g}{count(A)}(R) ](t).\lbMarker{count(A)} = \sum_{R(t')[g] \equiv t[g]}\lbMarker{R(t')} \]
% %\[ [ \aggregation{g}{count(A)}(R) ](t).\ubMarker{count(A)} = \sum_{R(t')[g] \matches t[g]}\ubMarker{R(t')} \]
% %
% %
% %\item Sum Aggregation without group by
% %\begin{align*}
% %[ & \aggregation{}{sum(A)}(R) ](t). \lbMarker{sum(A)} = \\ & \sum_{t' \in R}\{\lbMarker{R(t')}*R(t').\lbMarker{A}\}^+ + \{\ubMarker{R(t')}*R(t').\lbMarker{A}\}^-
% %\end{align*}
% %\begin{align*}
% %[ & \aggregation{}{sum(A)}(R) ](t). \ubMarker{sum(A)} = \\ & \sum_{t' \in R}\{\ubMarker{R(t')}*R(t').\ubMarker{A}\}^+ + \{\lbMarker{R(t')}*R(t').\ubMarker{A}\}^-
% %\end{align*}
% %
% %\item Sum Aggregation with group by
% %\[ [ \aggregation{g}{sum(A)}(R) ](t).\lbMarker{sum(A)} = \sum_{t' \in R, t[g] \in t'[g]}LB(R(t'))*R(t').\lbMarker{A} \]
% %\[ \forall_{a_i \in U } : [\projection_{U}(R)](t).\lbMarker{a_i} = \min_{t=t'[U]} R(t').\lbMarker{a_i} \]
% %\[ \forall_{a_i \in g } : [ \aggregation{g}{sum(A)}(R) ](t).\lbMarker{a_i} = \min_{[\projection_{g}(R)(t[g]) \matches R(t')[g]} R(t').\lbMarker{a_i} \]
% %\[ \forall_{a_i \in g } : [ \aggregation{g}{sum(A)}(R) ](t).\ubMarker{a_i} = \max_{[\projection_{g}(R)(t[g]) \matches R(t')[g]} R(t').\ubMarker{a_i} \]
% %\begin{align*}
% %[ & \aggregation{g}{sum(A)}(R) ](t). \lbMarker{sum(A)} = \\ & \sum_{R(t')[g] \equiv t[g]}\{\lbMarker{R(t')}*R(t').\lbMarker{A}\}^+ + \\ & \sum_{R(t')[g] \matches t[g]} \{\ubMarker{R(t')}*R(t').\lbMarker{A}\}^-
% %\end{align*}
% %\begin{align*}
% %[ & \aggregation{g}{sum(A)}(R) ](t). \ubMarker{sum(A)} = \\ & \sum_{R(t')[g] \matches t[g]}\{\ubMarker{R(t')}*R(t').\ubMarker{A}\}^+ + \\ & \sum_{R(t')[g] \equiv t[g]} \{\lbMarker{R(t')}*R(t').\ubMarker{A}\}^-
% %\end{align*}
% %
% %\end{enumerate}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsection{Examples}

The following example illustrates the application of the aggregation semantics we have defined in this section.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{Example}\label{ex:aggregation}
  Consider the relation shown in \Cref{fig:AU-aggregation} which records addresses (street, street number, number of inhabitants).
  Following~\cite{Yang:2015:LOA:2824032.2824055}, uncertain text fields are marked in red to indicate that their bound encompasses the whole domain.
  Street values $v$ in black are certain, i.e.,  $\lbMarker{v} = \bgMarker{v} = \ubMarker{v}$.
  We are uncertain about particular street numbers, number of inhabitants at certain addresses, and one street name. Furthermore, several tuples may represent more than one address. % Finally, we are uncertain about the street for the address represented by the second tuple.
  % Consider the aggregation query without group-by shown in \Cref{fig:AU-agg-example-no-GB}. We are calculating the number of inhabitants. In the \abbrBGW there are 7 inhabitants ($1 \cdot 1 + 2 \cdot 1 + 2 \cdot 2$).
  % As another example
  For the query shown in \Cref{fig:AU-agg-example-GB}
 consider the second result tuple (group \textit{State}). This tuple certainly exists since the 3rd tuple in the input appears twice in every world and its group-by value is certain. Thus, the count for group \textit{State} is at least two. The second input tuple could also belong to this group and, thus, the count could be $4$ (the upper bound).
 Note also the multiplicity of the first output tuple (group \textit{Canal}): \uv{1}{1}{2}.
 In the \abbrBGW the first two input tuples belong to this group.
 However, the second input tuple need not be in this group in all worlds, and in fact may not belong to any existing group.
 Thus, in some possible worlds this one \abbrAUDB tuple may represent 2 distinct output tuples.
\end{Example}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\subsection{Preservation of bounds}\label{sec:preserve-bounds-agg}

We are ready to state the main result of this section: our aggregation semantics for \abbrUAADBs is bound-preserving.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{Theorem}\label{theo:aggregation-preserves-bounds}
  Let $\query \defas \aggregation{\gbAttrs}{f(A)}(\rela)$ or $\query \defas \aggregation{}{f(A)}(\rela)$.
$\uaaN$-rel\-ational query semantics preserves bounds for $\query$.
  % and $\prel$ be an incomplete $\semK$-relation that is bound by an $\uaaK{\semK}$-relation $\rangeRel$. Then $\query(\rangeRel)$ bounds $\query(\prel)$.
\end{Theorem}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{proof}[Proof Sketch]
  The claim is proven by demonstrating that for every possible world $\rela$ of the input incomplete $\semN$-relation $\prel$ and a tuple matching $\TM$ based on which $\rangeRel$ bounds $\rela$, we can construct a tuple matching based on which $\query(\rangeRel)$ bounds $\query(\rela)$. For each aggregation result $\tup$ in $\rela$, we show that there is a result in $\query(\rangeRel)$ that bounds the values of $\tup$, because our aggregation semantics computes aggregation function results based on the minimum and maximum contribution of each possible input tuple, and group-by attribute bounds are generated by conservatively merging the group-by bounds of input tuples.
 See~\cite{techreport} for the full proof.
\end{proof}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Our main technical result follows from \Cref{theo:aggregation-preserves-bounds}\iftechreport{, \Cref{theo:set-difference-prese},}\ifnottechreport{,~\cite[Thm. 3]{techreport} (bound preservation for set difference)} and \Cref{lem:ra-plus-preserves-bounds}: % Our query semantics for $\raAgg$ queries preserves bounds.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{Corollary} %[Preservation of bounds for $\raAgg$]
  \label{cor:preservation-of-boun}
$\uaaN$-semantics preserves bounds for $\raAgg$.
  % Let $\query$ be an $\raAgg$ query and $\pdb$ an incomplete $\semN$-database that is bound by an $\uaaK{\semN}$-database $\rangeDB$. Then $\query(\rangeDB)$ bounds $\query(\pdb)$.
%  $$ \pdb \dbbounds \rangeDB \Rightarrow \query(\pdb) \dbbounds \query(\rangeDB)$$
\end{Corollary}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{proof}

% \end{proof}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "uaadb"
%%% End:


==> uaa-exprs.tex <==
%!TEX root = ./uaadb.tex
\section{Scalar Expressions}
\label{sec:expression}

%\BG{Only define $\leq$ and $=$ since $<$, $>$ and $\geq$ can then be defined using logical operators and these two}

%We now introduce a semantics for evaluating scalar expressions over a set of variables whose values are uncertain. %For that we first define expression syntax and semantics, then generalize to incomplete expressions, and finally introduce range-annotated values as a way to under- and over-approximate incomplete expressions. The techniques established in this section are then used to define \abbrUAADBs as relations whose values are range-annotated in \Cref{sec:uaa-range}.
% Recall that $\dataDomain$ denotes a universal domain of values.
\ifnottechreport{Consider a domain $\dataDomain$ that consists of $\mathbb{R}$ and the boolean values ($\bot$ and $\top$).}
\iftechreport{Recall that $\dataDomain$ denotes a domain of values. For this section we assume that $\dataDomain$ that consists of $\mathbb{R}$ and the boolean values ($\bot$ and $\top$).}
Furthermore, let $\mathbb{V}$ denote a countable set of variables.
 \iftechreport{ %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{Definition}[Expression Syntax]\label{def:expr-syntax}
	For any variable $x \in \mathbb{V}$, $x$ is an expression and for any constant $c \in \dataDomain$, $c$ is an expression.
	If $\sexpr_1$, $\sexpr_2$ and $\sexpr_3$ are expressions, then \ldots
    \begin{align*}
      &\sexpr_1 \wedge \sexpr_2
      &&\sexpr_1 \vee \sexpr_2
      && \neg \sexpr_1
      &&\sexpr_1 = \sexpr_2
      &&\sexpr_1 \neq \sexpr_2
      &&\sexpr_1 \leq \sexpr_2
    \end{align*}
    \begin{align*}
      &&\sexpr_1 + \sexpr_2
      &&\sexpr_1 \cdot \sexpr_2
      &&\frac{1}{\sexpr_1}
      &&\ifte{\sexpr_1}{\sexpr_2}{\sexpr_3}\\
    \end{align*}
	are also expressions. Given an expression $\sexpr$, we denote the variables in $\sexpr$ by $\vars(\sexpr)$.  \end{Definition}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
   }
   \ifnottechreport{
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{Definition}[Expression Syntax]\label{def:expr-syntax}
	For any variable $x \in \mathbb{V}$, $x$ is an expression and for any constant $c \in \dataDomain$, $c$ is an expression.
	If $\sexpr_1$, $\sexpr_2$ and $\sexpr_3$ are expressions, then \ldots\\[-6mm]
    \begin{align*}
      &\sexpr_1 \wedge \sexpr_2
      &&\sexpr_1 \vee \sexpr_2
      && \neg \sexpr_1
      &&\sexpr_1 = \sexpr_2
      &&\sexpr_1 \neq \sexpr_2
      &&\sexpr_1 \leq \sexpr_2
    \end{align*}\\[-11mm]
    \begin{align*}
      &&\sexpr_1 + \sexpr_2
      &&\sexpr_1 \cdot \sexpr_2
      &&\ifte{\sexpr_1}{\sexpr_2}{\sexpr_3}
    \end{align*}\\[-4mm]
	are also expressions. Given an expression $\sexpr$, we denote the variables of $\sexpr$ by $\vars(\sexpr)$.  % \end{Definition}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
     }
We will also use $\neq$, $\geq$, $<$, $-$, and $>$ since these operators can be defined using the expression syntax above, e.g., $e_1 > e_2 = \neg\, (e_1 \leq e_2)$. \iftechreport{Assuming that $\dataDomain$ contains negative numbers, subtraction can be expressed using addition and multiplication.}
For an expression $\sexpr$, given a valuation $\sval$ that maps variables from $\vars(\sexpr)$ to constants from $\dataDomain$, the expression evaluates to a constant \ifnottechreport{$\seval{e}{\sval}$} from $\dataDomain$. \ifnottechreport{The semantics of these expressions are standard (see \cite{techreport} for explicit definitions).}
\iftechreport{The semantics of expression evaluation is defined below.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{Definition}[Expression Semantics]\label{def:expr-semantics}
	Let $\sexpr$ be an expression. Given a valuation  $\sval: \vars(e) \rightarrow \dataDomain$, the result of expression $\sexpr$ over $\sval$ is denoted as $\seval{\sexpr}{\sval}$. Note that $\seval{\frac{1}{\sexpr}}{\sval}$ is undefined if $\seval{\sexpr}{\sval} = 0$. The semantics of expression is defined as shown below:
    \begin{align*}
      \seval{x}{\sval}                                                                 & \defas \sval(x)
                                                                                       & \seval{c}{\sval}                                    & \defas c &
      \seval{\neg \sexpr_1}{\sval}                                                     & \defas \neg \seval{\sexpr_1}{\sval}
    \end{align*}
    \begin{align*}
     \seval{e_1 \wedge e_2}{\sval}                                                     & \defas \seval{e_1}{\sval} \wedge \seval{e_2}{\sval} &
    \seval{e_1 \vee e_2}{\sval}                                                        & \defas \seval{e_1}{\sval} \vee \seval{e_2}{\sval}                                                       \\
                                                          \seval{e_1 + e_2}{\sval}     & \defas \seval{e_1}{\sval} + \seval{e_2}{\sval}                                                          &
	 % \seval{e_1 - e_2}{\sval}                                                        & \defas \seval{e_1}{\sval} - \seval{e_2}{\sval}
                                                                                         \seval{e_1 \cdot e_2}{\sval} & \defas \seval{e_1}{\sval} \cdot \seval{e_2}{\sval}  \\
     \seval{\frac{1}{e_1}}{\sval} &\defas \frac{1}{\seval{e_1}{\sval}}\\
	 \seval{e_1 = e_2}{\sval}                                                          & \defas \seval{e_1}{\sval} = \seval{e_2}{\sval}                                                          &
                                                         %                             & \seval{e_1 > e_2}{\sval}                            & \defas \seval{e_1}{\sval} > \seval{e_2}{\sval}    \\
	 \seval{e_1 \leq e_2}{\sval}                                                       & \defas \seval{e_1}{\sval} \leq \seval{e_2}{\sval}
                                                         %                             & \seval{e_1 \neq e_2}{\sval}                         & \defas \seval{e_1}{\sval} \neq \seval{e_2}{\sval} \\
      \end{align*}
      \begin{align*}
      \seval{\ifte{\sexpr_1}{\sexpr_2}{\sexpr_3}}{\sval}                               & \defas
                                                                                         \begin{cases}
                                                                                           \seval{\sexpr_2}{\sval} &\mathtext{if}\; \seval{\sexpr_1}{\sval}\\
                                                                                           \seval{\sexpr_3}{\sval} &\mathtext{otherwise}
                                                                                         \end{cases}
% \ifte{\seval{\sexpr_1}{\sval}}{\seval{\sexpr_2}{\sval}}{\seval{\sexpr_3}{\sval}}
    \end{align*}
\end{Definition}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Incomplete Expression Evaluation}\label{sec:expr-incomplete}

We now define evaluation of expressions over incomplete valuations, which are sets of valuations.
Each valuation in such a set, called a possible world, represents one possible input for the expression.
The semantics of expression evaluation are then defined using % the well-known
possible worlds semantics: the result of evaluating an expression $\sexpr$ over an incomplete valuation $\uval = \{ \sval_1, \ldots, \sval_n \}$
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\ifnottechreport{ denoted as $\seval{\sexpr}{\uval}$
is the set of results obtained by evaluating $\sexpr$ over each $\sval_i$ using deterministic expression evaluation semantics:
$\seval{\sexpr}{\uval} \defas \{ \seval{\sexpr}{\sval} \mid \sval \in \uval \}$.
Consider an expression $\sexpr \defas x+y$ and an incomplete valuation $\uval = \{ (x=1,y=4), (x=2,y=4), (x=1,y=5) \}$.
We get $\seval{\sexpr}{\uval} = \{ 1+4, 2+4, 1+5 \} = \{5,6\}$. }
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\iftechreport{
is the set of results obtained by evaluating $\sexpr$ over each $\sval_i$ using the deterministic expression evaluation semantics defined above.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{Definition}[Incomplete Expression Semantics]\label{def:incomplete-expr-sem}
An incomplete valuation $\uval$ is a set $\{ \sval_1, \ldots, \sval_n \}$ where each $\sval_i$ is a valuation.
The result of evaluating an expression $\sexpr$ over $\uval$ denoted as $\seval{\sexpr}{\uval}$ is:
$$\seval{\sexpr}{\uval} \defas \{ \seval{\sexpr}{\sval} \mid \sval \in \uval \}$$
% An incomplete expression evaluation is a valuation with a set of possible variable to value bindings $vars(e) \rightarrow \{\dataDomain\}$ and evaluates to a set of possible values from the domain $\varphi(e) \rightarrow \{\dataDomain\}$
\end{Definition}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{Example}
	Consider an expression $\sexpr \defas x+y$ and an incomplete valuation with possible bindings $\uval = \{ (x=1,y=4), (x=2,y=4), (x=1,y=5) \}$. Applying deterministic evaluation semantics for each of the three valuations from $\uval$ we get  $1+4=5$ ,$2+5=6$, and $1+5=6$. Thus, the possible outcomes of this expression under this valuation are: $\seval{\sexpr}{\uval} = \{5,6\}$.
\end{Example}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% The incomplete expression evaluation result can be obtained by performing conventional expression evaluating over each possible variable bindings and union their result.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\ifnottechreport{
\subsection{Range-Annotated Domains}\label{sec:range-dom}
}
\iftechreport{
\subsection{Range-Annotated Domains}\label{sec:range-dom}
}
We now define \textit{range-annotated values}, which are domain values that are annotated with an interval that bounds the value from above and below.
% values can only be annotated by either certain or uncertain, we assume a random total order for the categorical domain and annotate uncertain attributes using the lowest and largest value from the domain as the lower and upper bound.
% \BG{@Su: adapt notation as in the previous sections}
We define an expression semantics for valuations that maps variables to range-annotated values and then prove that if the input bounds an incomplete valuation, then the range-annotated output produced by this semantics bounds the possible outcomes of the incomplete expression.
% \BG{Following may be possible to omit:
% These results for evaluating expressions under uncertainty will then be utilized afterwards to define relations whose values stem from the annotated domain and which are used to bound the possible worlds of an incomplete database from below and above.}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{Definition}%[Range annotated domain]
  \label{def:range-domain}
Let $\dataDomain$ be a domain and let $\leq$ denote a total order over its elements. Then the \emph{range-annotated domain} $\rangeDom$ is defined as:
%
$$\left\{ \uv{\lbMarker{c}}{\bgMarker{c}}{\ubMarker{c}} \mid \lbMarker{c}, \bgMarker{c}, \ubMarker{c} \in \dataDomain \wedge \lbMarker{c} \leq \bgMarker{c} \leq \ubMarker{c} \right\}$$

  % a function $\dataDomain \rightarrow I$ where $I=\dataDomain^2$ denotes the highest and lowest possible value of the element. For an element $x \in \rangeDom$, we use $\ubMarker{x}$ to denote the upper bound and $\lbMarker{x}$ to denote the lower bound of the element.
\end{Definition}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

A value $c = \uv{\lbMarker{c}}{\bgMarker{c}}{\ubMarker{c}}$ from $\rangeDom$ encodes a value $\bgMarker{c} \in \dataDomain$ and two values ($\lbMarker{c}$ and $\ubMarker{c}$) that bound $\bgMarker{c}$ from below and above.
% To simplify presentation, we alternatively write a range-annotated element $(c_1, c_2, c_3) \in \rangeDom$ as $\uv{c_1}{c_2}{c_3}$.
%Given $c = \uv{c_1}{c_2}{c_3} \in \rangeDom$, we write $\lbMarker{c}$ to denote $c_1$, $\ubMarker{c}$ to denote $c_3$ and $\bgMarker{c}$ to denote $c_2$.
We call a value $c \in \rangeDom$  \emph{certain} if $\lbMarker{c}=\bgMarker{c}=\ubMarker{c}$.
Observe, that the definition requires that for any $c \in \rangeDom$ we have $\lbMarker{c} \leq \bgMarker{c} \leq \ubMarker{c}$.
% We also set constrain to the bounds so that the value must be in the bound $\lbMarker{x} \leq x \leq \ubMarker{x}$.
\iftechreport{
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{Example}
  For the boolean domain $\dataDomain=\{\bfalse,\btrue\}$ with order $\bfalse < \btrue$, the corresponding range annotated domain is:
  $$\rangeDom=\{\uv{\btrue}{\btrue}{\btrue},\uv{\bfalse}{\btrue}{\btrue},\uv{\bfalse}{\bfalse}{\btrue},\uv{\bfalse}{\bfalse}{\bfalse}\}$$
\end{Example}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
}
We use valuations that map the variables of an expression to elements from $\rangeDom$ % and use such valuations
to % encode
bound % on the possible values of
incomplete valuations.
%Instead of using a set of possible bindings to the variable from the original domain, we bind the uncertain variable to a single value from the interval annotated domain $\rangeDom$.

\iftechreport{
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{Definition}[Range-annotated valuation]\label{def:range-val}
Let $\sexpr$ be an expression. A \emph{range-annotated valuation} $\rval$ for $\sexpr$ is a mapping $\vars(\sexpr) \to \rangeDom$.
  % For an uncertain variable with a set of possible bindings $x=\{v_1,v_2,...,v_n\}$. And a binding to the annotated domain $x=v^I$. We call the binding as a sound bound iff the bound fully covers all possible outcomes of the original bindings $\lbMarker{x} \leq min(\{v_1,v_2,...,v_n\}) \wedge \ubMarker{x} \geq max(\{v_1,v_2,...,v_n\})$.
\end{Definition}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{Definition}% [Bounding valuations]
  \label{def:range-expr-bound}
  \ifnottechreport{A \emph{range-annotated valuation} $\rval$ for an expression $\sexpr$ is a mapping $\vars(\sexpr) \to \rangeDom$.}
  Given an incomplete valuation $\uval$ % for an expression $\sexpr$
  and  a range-annotated valuation $\rval$ for $\sexpr$,
  we say that $\rval$ bounds $\uval$ iff
  \begin{align*}
    \forall x \in \vars(\sexpr): \forall \sval \in \uval: \lbMarker{\rval(x)} \leq \sval(x) \leq \ubMarker{\rval(x)}\\
    \exists \sval \in \uval: \forall x \in \vars(\sexpr): \sval(x) = \bgMarker{\rval(x)}
  \end{align*}
  % For an uncertain variable with a set of possible bindings $x=\{v_1,v_2,...,v_n\}$. And a binding to the annotated domain $x=v^I$. We call the binding as a sound bound iff the bound fully covers all possible outcomes of the original bindings $\lbMarker{x} \leq min(\{v_1,v_2,...,v_n\}) \wedge \ubMarker{x} \geq max(\{v_1,v_2,...,v_n\})$.
\end{Definition}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\ifnottechreport{
Consider the incomplete valuation $\uval = \{(x=1),(x=2),(x=3)\}$. The range-annotated valuation  $x=\uv{0}{2}{3}$ is a bound for $\uval$, while $x=\uv{0}{2}{2}$ is not a bound.
}
\iftechreport{
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{Example}
Consider the incomplete valuation $\uval = \{(x=1),(x=2),(x=3)\}$. The range-annotated valuation  $x=\uv{0}{2}{3}$ is a bound for $\uval$, while $x=\uv{0}{2}{2}$ is not a bound.
  \end{Example}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\iftechreport{
\subsection{Range-annotated Expression Evaluation}\label{sec:range-expr-eval}
}
%
We now define a semantics for evaluating expressions over range-annotated valuations. We then demonstrate that this semantics preserves bounds.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{Definition}\iftechreport{[Range-annotated expression evaluation]}
  \label{def:range-expr-eval}
  Let $\sexpr$ be an expression. Given a range valuation $\rval: \vars(e) \rightarrow \rangeDom$,
we define % $\bgMarker{\rval}$ as the valuation
$\bgMarker{\rval}(x) \defas \bgMarker{\rval(x)}$.
  The result of expression $\sexpr$ over $\rval$ denoted as $\seval{\sexpr}{\rval}$ is defined as:
    \begin{align*}
      \seval{x}{\rval} &\defas \uv{\lbMarker{\rval(x)}}{\bgMarker{\rval(x)}}{\ubMarker{\rval(x)}} &
      \seval{c}{\rval} &\defas \uv{c}{c}{c}
    \end{align*}
    \ifnottechreport{
    For any of the following expressions we define $\bgMarker{\seval{e}{\rval}} \defas \seval{e}{\bgMarker{\rval}}$. Let $\seval{e_1}{\rval} = a$, $\seval{e_2}{\rval} = b$, and $\seval{e_3}{\rval} = c$. All expressions omitted below are defined point-wise (e.g., $\lbMarker{\seval{e_1 + e_2}{\rval}} \defas \lbMarker{a} + \lbMarker{b}$).
%
   \begin{align*}
%%%%%%%%%%%%%%%%%%%%
% 	 \lbMarker{\seval{e_1 \wedge e_2}{\rval}} &\defas \lbMarker{a} \wedge \lbMarker{b} &
% 	 \ubMarker{\seval{e_1 \wedge e_2}{\rval}} &\defas \ubMarker{a} \wedge \ubMarker{b}\\
% %%%%%%%%%%%%%%%%%%%%
%       \lbMarker{\seval{e_1 \vee e_2}{\rval}} &\defas \lbMarker{a} \vee \lbMarker{b} &
%       \ubMarker{\seval{e_1 \vee e_2}{\rval}} &\defas \ubMarker{a} \vee \ubMarker{b} \\
%%%%%%%%%%%%%%%%%%%%
      \lbMarker{\seval{\neg e_1}{\rval}} &\defas \neg\, \ubMarker{a} &
      \ubMarker{\seval{\neg e_1}{\rval}} &\defas \neg\, \lbMarker{a}
%%%%%%%%%%%%%%%%%%%%
      % \lbMarker{\seval{e_1 + e_2}{\rval}} &\defas \lbMarker{a} + \lbMarker{b} &
      % \ubMarker{\seval{e_1 + e_2}{\rval}} &\defas \ubMarker{a} + \ubMarker{b}
    \end{align*}\\[-10mm]
    \begin{align*}
%%%%%%%%%%%%%%%%%%%%
      \lbMarker{\seval{e_1 \cdot e_2}{\rval}}                                                                                         &\defas \min(\;\;\ubMarker{a} \cdot \ubMarker{b},\;\;
                      \ubMarker{a} \cdot \lbMarker{b},\;\;
                      \lbMarker{a} \cdot \ubMarker{b},\;\;
                      \lbMarker{a} \cdot \lbMarker{b}\;\;)\\
      \ubMarker{\seval{e_1 \cdot e_2}{\rval}}                                                                       &
      \defas \max(\;\;\ubMarker{a} \cdot \ubMarker{b},\;\;
                      \ubMarker{a} \cdot \lbMarker{b},\;\;
                      \lbMarker{a} \cdot \ubMarker{b},\;\;
                      \lbMarker{a} \cdot \lbMarker{b}\;\;)
     %%%%%%%%%%%%%%%%%%%%
    \end{align*}\\[-10mm]
    \begin{align*}
      \lbMarker{\seval{e_1 \leq e_2}{\rval}} &\defas \ubMarker{a} \leq \lbMarker{b} &
 \lbMarker{\seval{e_1=e_2}{\rval}} &\defas \ubMarker{a}=\lbMarker{b} \wedge \ubMarker{b}=\lbMarker{a} \\
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 \ubMarker{\seval{e_1 \leq e_2}{\rval}} &\defas \lbMarker{a} \leq \ubMarker{b} &
                                                                                                 \ubMarker{\seval{e_1=e_2}{\rval}} &\defas \lbMarker{a} \leq \ubMarker{b} \wedge \lbMarker{b} \leq \ubMarker{a}
 % \ubMarker{a}>\lbMarker{b} \wedge \lbMarker{a}<\lbMarker{b} \vee \ubMarker{a}>\ubMarker{b} \wedge \lbMarker{a}<\ubMarker{b} \\
    \end{align*}\\[-10mm]
    \begin{align*}
\lbMarker{\seval{\ifte{e_1}{e_2}{e_3}}{\rval}} &\defas
 \begin{cases}
\lbMarker{b} & \text{if } \lbMarker{a}= \ubMarker{a}=\btrue \\
\lbMarker{c} & \text{if } \lbMarker{a}= \ubMarker{a}=\bfalse \\
 \min(\lbMarker{b},\lbMarker{c}) & \text{else}
\end{cases}\\
      \ubMarker{\seval{\ifte{e_1}{e_2}{e_3}}{\rval}} &\defas
 \begin{cases}
 \ubMarker{b} & \text{if } \lbMarker{a}= \ubMarker{a}=\btrue \\
\ubMarker{c} & \text{if } \lbMarker{a}= \ubMarker{a}=\bfalse \\
\max(\ubMarker{b},\ubMarker{c}) & \text{else}
\end{cases}
    \end{align*}
    }
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \iftechreport{
Note that $\seval{\frac{1}{\sexpr}}{\rval}$ is undefined if $\lbMarker{\seval{\sexpr}{\rval}} \leq 0$ and $\ubMarker{\seval{\sexpr}{\rval}} \geq 0$, because then $\rval$ may bound a valuation $\sval$ where $\seval{\sexpr}{\sval} = 0$.
      For any of the following expressions we define $\bgMarker{\seval{e}{\rval}} \defas \seval{e}{\bgMarker{\rval}}$. Let $\seval{e_1}{\rval} = a$, $\seval{e_2}{\rval} = b$, and $\seval{e_3}{\rval} = c$. Then,
      \begin{align*}
%%%%%%%%%%%%%%%%%%%%
	 \lbMarker{\seval{e_1 \wedge e_2}{\rval}} &\defas \lbMarker{a} \wedge \lbMarker{b} &
	 \ubMarker{\seval{e_1 \wedge e_2}{\rval}} &\defas \ubMarker{a} \wedge \ubMarker{b}\\
%%%%%%%%%%%%%%%%%%%%
      \lbMarker{\seval{e_1 \vee e_2}{\rval}} &\defas \lbMarker{a} \vee \lbMarker{b} &
      \ubMarker{\seval{e_1 \vee e_2}{\rval}} &\defas \ubMarker{a} \vee \ubMarker{b} \\
%%%%%%%%%%%%%%%%%%%%
      \lbMarker{\seval{\neg e_1}{\rval}} &\defas \neg\, \ubMarker{a} &
      \ubMarker{\seval{\neg e_1}{\rval}} &\defas \neg\, \lbMarker{a} \\
%%%%%%%%%%%%%%%%%%%%
      \lbMarker{\seval{e_1 + e_2}{\rval}} &\defas \lbMarker{a} + \lbMarker{b} &
      \ubMarker{\seval{e_1 + e_2}{\rval}} &\defas \ubMarker{a} + \ubMarker{b}
    \end{align*}\\[-10mm]
    \begin{align*}
%%%%%%%%%%%%%%%%%%%%
      \lbMarker{\seval{e_1 \cdot e_2}{\rval}}                                                                                         &\defas \min(\ubMarker{a} \cdot \ubMarker{b},\ubMarker{a} \cdot \lbMarker{b},\lbMarker{a} \cdot \ubMarker{b},\lbMarker{a} \cdot \lbMarker{b})\\
      \ubMarker{\seval{e_1 \cdot e_2}{\rval}}                                                                       &\defas \max(\ubMarker{a} \cdot \ubMarker{b},\ubMarker{a} \cdot \lbMarker{b},\lbMarker{a} \cdot \ubMarker{b},\lbMarker{a} \cdot \lbMarker{b})\\
      %%%%%%%%%%%%%%%%%%%%
                                                                                                                     \lbMarker{\seval{\frac{1}{e_1}}{\rval}}                                                                                         &\defas \frac{1}{\ubMarker{a}})\\
      \ubMarker{\seval{\frac{1}{e_1}}{\rval}}                                                                       &\defas \frac{1}{\lbMarker{a}}
      %%%%%%%%%%%%%%%%%%%%
    \end{align*}
    \begin{align*}
      \lbMarker{\seval{a \leq b}{\rval}} &\defas \ubMarker{a} \leq \lbMarker{b} &
 \ubMarker{\seval{a \leq b}{\rval}} &\defas \lbMarker{a} \leq \ubMarker{b} \\
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\lbMarker{\seval{a=b}{\rval}} &\defas (\ubMarker{a}=\lbMarker{b} \wedge \ubMarker{b}=\lbMarker{a} ) &
                                                                                                 \ubMarker{\seval{a=b}{\rval}} &\defas \lbMarker{a} \leq \ubMarker{b} \wedge \lbMarker{b} \leq \ubMarker{a}
 % \ubMarker{a}>\lbMarker{b} \wedge \lbMarker{a}<\lbMarker{b} \vee \ubMarker{a}>\ubMarker{b} \wedge \lbMarker{a}<\ubMarker{b} \\
    \end{align*}\\[-10mm]
    \begin{align*}
\lbMarker{\seval{\ifte{e_1}{e_2}{e_3}}{\rval}} &\defas
 \begin{cases}
\lbMarker{b} & \text{if } \lbMarker{a}= \ubMarker{a}=\btrue \\
\lbMarker{c} & \text{if } \lbMarker{a}= \ubMarker{a}=\bfalse \\
 \min(\lbMarker{b},\lbMarker{c}) & \text{else}
\end{cases}\\
      \ubMarker{\seval{\ifte{e_1}{e_2}{e_3}}{\rval}} &\defas
 \begin{cases}
 \ubMarker{b} & \text{if } \lbMarker{a}= \ubMarker{a}=\btrue \\
\ubMarker{c} & \text{if } \lbMarker{a}= \ubMarker{a}=\bfalse \\
\max(\ubMarker{b},\ubMarker{c}) & \text{else}
\end{cases}
    \end{align*}
      }
\end{Definition}
% Comparison and boolean operators are defined as:
% \begin{enumerate}

% \item \[\ubMarker{(a>b)} = \ubMarker{a}>\lbMarker{b}\] \\
% \[\lbMarker{(a>b)} = \lbMarker{a}>\ubMarker{b}\]

% \item \[\ubMarker{(a=b)} = \ubMarker{a}>\lbMarker{b} \wedge \lbMarker{a}<\lbMarker{b} \vee \ubMarker{a}>\ubMarker{b} \wedge \lbMarker{a}<\ubMarker{b}\] \\

% \[\lbMarker{(a=b)} = (\ubMarker{a}=\lbMarker{b} \wedge \ubMarker{b}=\lbMarker{a} )\] \\

% \item \[ \ubMarker{(p \wedge q)} = \ubMarker{p} \wedge \ubMarker{q} \]
% \[ \lbMarker{(p \wedge q)} = \lbMarker{p} \wedge \lbMarker{q} \]
% \item \[ \ubMarker{(p \vee q)} = \ubMarker{p} \vee \ubMarker{q} \]
% \[ \lbMarker{(p \vee q)} = \lbMarker{p} \vee \lbMarker{q} \]
% \end{enumerate}
% For arithmetic and conditional scalar expressions $a$ and $b$, we define expression evaluation in $\rangeDom$ as follows:
% \begin{enumerate}
% 	\item $ \ubMarker{(a+b)} = \ubMarker{a} + \ubMarker{b} $ \\
% 	$ \lbMarker{(a+b)} = \lbMarker{a} + \lbMarker{b} $
%     \item $ \ubMarker{(a-b)} = \ubMarker{a} - \lbMarker{b} $ \\
% 	$ \lbMarker{(a-b)} = \lbMarker{a} - \ubMarker{b} $
% 	\item $ \ubMarker{(a \cdot b)} = max(\ubMarker{a} \cdot \ubMarker{b},\ubMarker{a} \cdot \lbMarker{b},\lbMarker{a} \cdot \ubMarker{b},\lbMarker{a} \cdot \lbMarker{b}) $ \\
% 	$ \lbMarker{(a \cdot b)} = min(\ubMarker{a} \cdot \ubMarker{b},\ubMarker{a} \cdot \lbMarker{b},\lbMarker{a} \cdot \ubMarker{b},\lbMarker{a} \cdot \lbMarker{b}) $
% \]
% \end{enumerate}

\iftechreport{
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Preservation of Bounds}\label{sec:range-expr-eval-preserves-bounds}
}

Assuming that an input range-annotated valuation bounds an incomplete valuation, we need to prove that the output of range-annotated expression evaluation also  bounds the possible outcomes. % produced for the incomplete valuation.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{Definition}% [Bounding sets of values]
  \label{def:bounding-vals}
  A value $c \in \rangeDom$ % is said to
  bounds a set of values $S \subseteq \dataDomain$ if: %  = \{c_1, \ldots, c_n\}$ % from $\dataDomain$
  % if:
  \begin{align*}
    &\forall c_i \in S: \lbMarker{c} \leq c_i \leq \ubMarker{c}
    &&\exists c_i \in S: c_i = \bgMarker{c}
  \end{align*}
\end{Definition}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{Theorem}% [Bound Preservation]
  \label{theo:expr-bound}
  % Let $\sexpr$ be an expression, $\uval$ an incomplete valuation for $\sexpr$, and $\rval$ a range-annotated valuation % for $\sexpr$
  % that bounds $\uval$,
Let $\rval$ be a range-annotated valuation that bounds an incomplete valuation $\sexpr$ for an expression $e$,
  then $\seval{\sexpr}{\rval}$ bounds $\seval{\sexpr}{\uval}$.
\end{Theorem}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\ifnottechreport{
  \begin{proof}[Proof Sketch]
Proven by straightforward induction over the structure of formulas. We present the full proof in \cite{techreport}.
  \end{proof}
}
\iftechreport{
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{proof}
  We prove this theorem through induction over the structure of an expression under the assumption that $\rval$ bounds $\uval$.

\proofpara{Base case}
If $e \defas c$ for a constant $c$, then $\lbMarker{e} = \bgMarker{e} = \ubMarker{e} = c$ which is also the result of $e$ in any possible world of $\uval$. If $e \defas x$ for a variable $x$, then since $\rval$ bounds $\uval$, the value of $x$ in any possible world is bounded by $\rval(x)$.

\proofpara{Induction step}
Assume that for expressions $e_1$, $e_2$, and $e_3$, we have that their results under $\uval$ are bounded by their result under $\rval$:

\begin{align*}
\forall i \in \{1,2,3\}: \forall c \in \seval{e_i}{\uval}: \lbMarker{\seval{e_i}{\rval}} \leq c \leq \ubMarker{\seval{e_i}{\rval}}\\
\exists \sval \in \uval: \forall i \in \{1,2,3\}: \bgMarker{\seval{e_i}{\rval}} = \seval{e_i}{\sval}
\end{align*}
Note that the second condition trivially holds since $\bgMarker{\seval{e}{\rval}}$ was defined as applying deterministic expression semantics to $\bgMarker{\rval}$. We, thus, only have to prove  that the lower and upper bounds are preserved for all expressions $e$ that combine these expressions using one of the scalar, conditional, or logical operators.

\proofpara{$e \defas e_1 + e_2$}
Inequalities are preserved under addition. Thus, for any $\sval \in \uval$ we have $\lbMarker{\seval{e_1}{\rval}} + \lbMarker{\seval{e_2}{\rval}} \leq \seval{e_1}{\sval} + \seval{e_2}{\sval} \leq \ubMarker{\seval{e_1}{\rval}} + \ubMarker{\seval{e_2}{\rval}}$.

\proofpara{$e \defas e_1 \cdot e_2$}
We distinguish sixteen cases based on which of $\lbMarker{\seval{e_1}{\rval}}$, $\lbMarker{\seval{e_2}{\rval}}$, $\ubMarker{\seval{e_1}{\rval}}$, and $\lbMarker{\seval{e_2}{\rval}}$ are negative. For instance, if all numbers are positive then clearly $\lbMarker{\seval{e_1}{\rval}} \cdot \lbMarker{\seval{e_2}{\rval}} \leq \seval{e_1}{\sval} \cdot \seval{e_2}{\sval}$. While there are sixteen cases, there are only four possible combinations of lower and upper bounds we have to consider. Thus, if we take the minimal (maximal) value across all these cases, we get a lower (upper) bound on $e$.

\proofpara{$e \defas \frac{1}{e_1}$}
For any pair of numbers $c_1$ and $c_2$ that are either both positive or both negative, we have $c_1 \leq c_2$ implies $\frac{1}{c_1} \geq \frac{1}{c_2}$. Thus, $\frac{1}{\ubMarker{a}}$ is an upper bound on $\frac{1}{c}$ for any $c$ bound by $a$. Analog, $\frac{1}{\lbMarker{a}}$ is an upper bound.

\proofpara{$e \defas e_1 \wedge e_2$ and $e \defas e_1 \vee e_2$}
Both $\vee$ and $\wedge$ are monotone in their arguments wrt. the order $F \ordB T$. Thus, applying these operations to combine lower (upper) bounds preserves these bounds.

\proofpara{$e \defas \neg\,e_1$}
We distinguish three cases: (i) $\seval{e_1}{\sval} = \bfalse$ for all $\sval \in \uval$; (ii)$\seval{e_1}{\sval} = \btrue$ for some $\sval \in \uval$ and $\seval{e_1}{\sval} = \bfalse$ for some $\sval \in \uval$; and (iii) $\seval{e_1}{\sval} = \bfalse$ for all $\sval \in \uval$. In case (i) for $\rval$ to bound the input either $\seval{e_1}{\rval} = \uv{\bfalse}{\bfalse}{\bfalse}$ in which case $\seval{e}{\rval} = \uv{\btrue}{\btrue}{\btrue}$ or $\seval{e_1}{\rval} = \uv{\bfalse}{\bfalse}{\btrue}$ and $\seval{r}{\rval} = \uv{\bfalse}{\btrue}{\btrue}$. We have $\seval{e}{\sval} = \btrue$ for all $\sval \in \uval$ and, thus, in either case $\seval{e}{\rval}$ bounds $\seval{e}{\uval}$. In case (ii), $\lbMarker{\seval{e}{\rval}} = \bfalse$ and $\ubMarker{\seval{e}{\rval}} = \btrue$ which trivially bound $\seval{e}{\uval}$. The last case is symmetric to (i).

\proofpara{$e \defas e_1 \leq e_2$}
Recall that $\bfalse \leq \btrue$.  $e_1 \leq  e_2$ is guaranteed to evaluate to true in every possible world if the upper bound of $e_1$ is lower than or equal to the lower bound of $e_2$. In this case it is safe to set $\lbMarker{\seval{e}{\rval}} = \btrue$. Otherwise, there may exist a possible world where $e_1 \leq e_2$ evaluates to false and we have to set $\lbMarker{\seval{e}{\rval}} = \bfalse$. Similarly, if the lower bound of $e_1$ is larger than the upper bound of $e_2$ then $e_1 \leq e_2$ evaluates to false in every possible world and $\ubMarker{\seval{e}{\rval}} = \bfalse$ is an upper bound. Otherwise, there may exist a world where $e_1 \leq e_2$ holds and we have to set $\ubMarker{\seval{e}{\rval}} = \btrue$.

\proofpara{$\ifte{e_1}{e_2}{e_3}$}
When $e_1$ is certainly true ($\lbMarker{\seval{e_1}{\rval}} = \ubMarker{\seval{e_1}{\rval}} = \btrue$) or certainly false ($\lbMarker{\seval{e_1}{\rval}} = \ubMarker{\seval{e_1}{\rval}} = \bfalse$) then the bounds $e_2$ (certainly true) or $e_3$ (certainly false) are bounds for $e$. Otherwise, $e$ may evaluate to $e_2$ in some worlds and to $e_3$ in others. Taking the minimum (maximum) of the bounds for $e_2$ and $e_3$ is guaranteed to bound $e$ from below (above) in any possible world.

% 	\begin{itemize}
% 		% \item For operation $a+b$, by definition $\lbMarker{a} \leq a \leq \ubMarker{a}$ and $\lbMarker{b} \leq b \leq \ubMarker{b}$. So $\lbMarker{a}+\lbMarker{b} \leq a+b \leq \ubMarker{a}+\ubMarker{b}$. So the result is bounded.
% 	 	% \item For operation $a-b$, by definition $\lbMarker{a} \leq a \leq \ubMarker{a}$ and $\lbMarker{b} \leq b \leq \ubMarker{b}$. So $\lbMarker{a}-\ubMarker{b} \leq a-b \leq \ubMarker{a}-\lbMarker{b}$. So the result is bounded.
% 	 	% \item For operation $a \cdot b$, by definition $\lbMarker{a} \leq a \leq \ubMarker{a}$ and $\lbMarker{b} \leq b \leq \ubMarker{b}$. If $\lbMarker{a}>0$ and $\lbMarker{b}>0$ then $\lbMarker{a} \cdot \lbMarker{b} \leq a \cdot b$. Else if $\ubMarker{a}<0$ and $\ubMarker{b}<0$ then $\ubMarker{a} \cdot \ubMarker{b} \leq a \cdot b$. Else if $\lbMarker{a}>0$ and $\lbMarker{b}<0$ then $\ubMarker{a} \cdot \lbMarker{b} \leq a \cdot b$ or $\ubMarker{b} \cdot \lbMarker{a} \leq a \cdot b$. Same apply to the upper bounds symmetrically. So the result is bounded.
% 	 	\item For operation $a>b$, by definition $\lbMarker{a} \leq a \leq \ubMarker{a}$ and $\lbMarker{b} \leq b \leq \ubMarker{b}$. So it is possible for $a>b$ to be true iff $\ubMarker{a} > \lbMarker{b}$. It is possible for $a>b$ to be false iff $!(\lbMarker{a} > \ubMarker{b})$. So the result is bounded.
% 	 	\item For operation $a=b$, It is possible for $a=b$ to be true iff the bounds of the two inputs are overlapped. It is possible for $a=b$ to be false iff two values are not certainly equal. So the result is bounded.
% 	 	% \item For operation $a \wedge b$, It is possible for $a \wedge b$ to be true iff $\ubMarker{a}$ and $\ubMarker{b}$ is true. It is possible for $a \wedge b$ to be false iff $\lbMarker{a}$ or $\lbMarker{b}$ is false. So the result is bounded.
% 	 	% \item For operation $a \vee b$, It is possible for $a \vee b$ to be true iff $\ubMarker{a}$ or $\ubMarker{b}$ is true. It is possible for $a \wedge b$ to be false iff $\lbMarker{a}$ and $\lbMarker{b}$ is false. So the result is bounded.
% 	 	\end{itemize}

% \SF{Feels the boolean operators proofs are little shaky, maybe use contradictions?}

We conclude that the result of range-annotated expression evaluation under $\rval$ which bounds an incomplete valuation $\uval$ bounds the result of incomplete expression evaluation for any expression $e$.
% our expression evaluation model is bounded by the fact that any expression is recursively start with the base case which is bounded, and all the operator result is bounded given the input is bounded.
\end{proof}
}

Conditional range-annotated expressions are bound-preserving for any totally-ordered domain. \iftechreport{
We can add support for additional scalar operations as long as a bound-preserving evaluation semantics can be defined.
  Important classes of scalar operations are operations that preserve the order over the domain, i.e., for any domain values $a < b$ and $c < d$ which $a \diamond b $. For instance, this is the case for addition over natural numbers. For any such operation, point-wise application to range-annotated domain values is bound preserving. }
For categorical values where no sensible order can be defined, we impose an arbitrary order.
\iftechreport{Note that in the worst-case, we can just annotate a value with the range covering the whole domain to indicate that it is completely uncertain.}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "uaadb"
%%% End:


==> uaa-rels.tex <==
%!TEX root=./uaadb.tex
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{\abbrUAADBs}
\label{sec:uaa-range}

We define \termUAADBs (\abbrUAADBs) as a special type of $\semK$-relation over range-annotated domains and demonstrate how to bound an incomplete $\semK$-relation using this model.
Afterwards, we define a metric for how precise the bounds of an incomplete $\semK$-database encoded by an \abbrUAADB are, and  define a query semantics for \abbrUAADBs  that preserves bounds.
We limit the discussion to semiring $\semN$ (bag semantics). See~\cite{techreport} for the generalization to other semirings including $\semB$ (set semantics). % (semirings whose elements form a lattice structure).
% For the general construction  that works for any l-semiring (a semiring whose elements form a lattice structure) including $\semB$ (set semantics) see~\cite{techreport}.
% }
% \iftechreport{
% \abbrUAADBs are definedfor any l-semiring (a semiring whose elements form a lattice structure) including $\semB$ (set semantics), $\semN$ (bag semantics), security clearance annotations, and various types of provenance.
% }

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{$\uaaN$-relations}\label{sec:uaadbs}

In addition to allowing for range-annotated values, \abbrUAADBs also differ from \abbrUADBs in that they encode an upper bound of the possible annotation of each tuple. We use $\semqN$ annotations to encode for each tuple: a lower bound on the certain multiplicity of the tuple, the  multiplicity of the tuple in the \abbrBGW, and an over-approximation of the tuple's possible multiplicity.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{Definition}% [Tuple-level Annotations]
  \label{def:uaa-tuple-annot}
The % level
range-annotated multiplicity domain $\uaaDomN$ is defined as:\\[-6mm]
%
  $$\{ \ut{\lbMarker{k}}{k}{\ubMarker{k}} \mid \lbMarker{k}, k, \ubMarker{k} \in \semN \wedge \lbMarker{k} \leq k \leq \ubMarker{k} \}$$
We use $\uaaN$ to denote semiring $\semqN$ restricted to elements from $\uaaDomN$.
  \end{Definition}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

  % Similar to the range-annotated domain,
  % A value $\ut{\lbMarker{k}}{\bgMarker{k}}{\ubMarker{k}}$ from $\uaaN$ encodes an element from $\semN$ and two elements ($\lbMarker{k}$ and $\ubMarker{k}$) that bound the element from below and above.
  % Given an
  % $\uaaN$-element $k = \ut{k_1}{k_2}{k_3}$ we define
  % $\lbMarker{k} = k_1$, $\bgMarker{k} = k_2$, and $\ubMarker{k} = k_3$.
  Note that $\uaaN$ is a semiring since when combining two elements of
  $\uaaN$ with $\addOf{\semqN}$ and $\multOf{\semqN}$, the result
  $\ut{\lbMarker{k}}{\bgMarker{k}}{\ubMarker{k}}$ fulfills the requirement $\lbMarker{k} \leq \bgMarker{k} \leq \ubMarker{k}$. This is
  the case because  addition and multiplication in $\semN$ preserve
   order~\cite{FH19}, and these operations in $\semqN$ are pointwise
  application of $\addN$ and $\multN$. % , e.g.,
  % $\ut{\lbMarker{k}}{k}{\ubMarker{k}} \addOf{\semqN} \ut{\lbMarker{l}}{l}{\ubMarker{l}} = \ut{\lbMarker{l} \addN \lbMarker{l}}{k \addN l}{\ubMarker{k}
  % \addN \ubMarker{l}}$ and
  % $k_1 \ordN k_2 \wedge k_3 \ordN k_4 \Rightarrow k_1 \addN k_3 \ordN k_2 \addN
  % k_4$ for any $k_1, k_2, k_3, k_4 \in \semN$.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \begin{Definition}% [$\uaaN$-relations]
    \label{def:uaa-rels}
% Given a range-annotated data domain $\rangeDom$,
A $\uaaN$-relation of arity $n$ is a function $\rangeRel: \rangeDom^n \rightarrow \uaaN$ with finite support $\{ \rangeTup \mid \rangeRel(\rangeTup) \neq \ut{0}{0}{0} \}$.
\end{Definition}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \BGdel{DONT THINK WE USE THIS UNTIL MUCH LATER WHERE WE EXPLAIN IT AGAIN ANYWAYS: As a notational convenience we show certain values, i.e., values $c \in \rangeDom$ where $\lbMarker{c} = \bgMarker{c} = \ubMarker{c} = c'$, as the deterministic value $c'$ they encode.}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Extracting \capitalBGW}\label{sec:uaab-get-bgw}

$\uaaN$-relations permit multiple tuples with identical values in the \termBGW (\abbrBGW). % \abbrBG values.
We extract the \termBGW encoded by a $\uaaN$-relation by grouping tuples based on their \abbrBG values and summing up their \abbrBG multiplicities.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{Definition}\label{def:bool-to-K}
We lift operator $\bgName$ from values to tuples: $\bgName: \rangeDom^n \to \dataDomain^n$, i.e., given an \abbrUAADB tuple $\rangeTup = \tuple{c_1, \ldots, c_n}$, % we define
$\bgOf{\rangeTup} \defas \tuple{\bgMarker{c_1}, \ldots, \bgMarker{c_n}}$. For a  $\uaaN$-relation $\rangeRel$, $\bgOf{\rangeRel}$, the \abbrBGW encoded by $\rangeRel$, is then defined as:\\[-5mm]
%
$$\bgOf{\rangeRel}(\tup) \defas \sum_{\bgOf{\rangeTup} = \tup} \bgOf{\left(\rangeRel(\rangeTup)\right)}$$
%  The corresponding $\uaak{\semN}$-relation  $D_{bg}=\{t \rightarrow \sum_{BG(\rangeTup)=t} \rangeTup.k\}$.
\end{Definition}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{Example}\label{ex:audb-instance}
\Cref{table:UAAR_inst} shows an instance of a $\uaaN$-relation $\rela$ where each attribute is a triple showing the lower bound, \termBG, and upper bound of the value. Each tuple is annotated by a triple showing the lower multiplicity bound, \termBG multiplicity, and the upper multiplicity bound of the tuple. % Since this is a $\uaaN$ relation, the annotations encode multiplicities of tuples.
For example, the first tuple represents a tuple $\tuple{1,1}$ that appears at least twice in every possible world (its lower multiplicity bound  is $2$), appears twice in the \abbrBGW, and appears no more than thrice in any world.
	\Cref{table:UAAR_bg} shows the \abbrBGW encoded by this \abbrUAADB which is computed by summing up the multiplicities of tuples with identical \abbrBG values. For instance, the first two tuples both represent tuple $\tuple{1,1}$ in the \abbrBGW and their annotations sum up to $5$ (i.e., the tuple $\tuple{1,1}$ appears five times).
  Conversely, the first two tuples of $\db_2$ match different \abbrUAADB tuples.
\end{Example}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[t]
	\centering

    \begin{minipage}{0.465\linewidth}
	\begin{subtable}{\linewidth}
	\centering
	\begin{tabular}{ c|cc}
      \textbf{A}  & \textbf{B}  & \underline{\semqN} \\
      				\cline{1-2}
		$\uv{1}{1}{1}$ & $\uv{1}{1}{1}$ & \ut{2}{2}{3}\\
		$\uv{1}{1}{1}$ & $\uv{1}{1}{3}$ & \ut{2}{3}{3}\\
		$\uv{1}{2}{2}$ & $\uv{3}{3}{3}$ & \ut{1}{1}{1}\\
	\end{tabular}
	\caption{Example \abbrUAADB instance}
	\label{table:UAAR_inst}
	\end{subtable}
  \end{minipage}
  \begin{minipage}{0.505\linewidth}
	\begin{subtable}{\linewidth}
	\centering
	% \begin{tabular}{ c|cc}
	% 	\textbf{A}  & \textbf{B}  & \underline{$\semN$}  \\
	% 	\cline{1-2}
	% 	$1$ & $1$ & 5\\
	% 	$2$ & $3$ & 1\\
        %    \end{tabular}
    \begin{minipage}{0.490\linewidth}
      \centering
    \underline{$\db_1$}                                                                           \\
    	\begin{tabular}{lc|cc}
                               & \textbf{A}                 & \textbf{B} & \underline{$\semN$}    \\
		\cline{2-3}
$\tup_1$                       & $1$                        & $1$        & 5                      \\
$\tup_2$                       & $2$                        & $3$        & 1                      \\
	\end{tabular}
  \end{minipage}
  \begin{minipage}{0.49\linewidth}
    \centering
    \underline{$\db_2$}                                                                           \\
    \begin{tabular}{lc|cc}
                               & \textbf{A}                 & \textbf{B} & \underline{$\semN$}    \\
		\cline{2-3}
 $\tup_3$                      & $1$                        & $1$        & 2                      \\
 $\tup_4$                      & 1                          & 3          & 2                      \\
$\tup_5$                       & $2$                        & $3$        & 1                      \\
	\end{tabular}
  \end{minipage}
  	\caption{Worlds $\db_1$ (\abbrBGW) and $\db_2$}
	\label{table:UAAR_bg}
	\end{subtable}
  \end{minipage}\\[-3mm]
	\caption{Example \abbrUAADB relation and two worlds it bounds}
  \label{table:UAAR_overall}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{figure}[ht]
%   \BG{F and T should be introduced beforehand}
% 	\centering
% 	\begin{subtable}{0.4\linewidth}
% 	\centering
% 	\caption{R-D1}
% 	\begin{tabular}{ |c|c|l}
% 				\cline{1-2}
% 		\textbf{A}  & \textbf{B}  &  \\
% 		\cline{1-2}
% 		1 & 1 & 2\\
% %				\cline{1-3}
% 		1 & 2 & 3\\
% %				\cline{1-3}
% 		2 & 3 & 1\\
% 				\cline{1-2}
% 	\end{tabular}
% 	\end{subtable}
% 	\begin{subtable}{0.4\linewidth}
% 	\centering
% 	\caption{R-D2}
% 	\begin{tabular}{ |c|c|l}
% 				\cline{1-2}
% 		\textbf{A}  & \textbf{B}  &  \\
% 		\cline{1-2}
% 		1 & 1 & 3\\
% %				\cline{1-3}
% 		1 & 2 & 2\\
% %				\cline{1-3}
% 		1 & 3 & 2\\
% 				\cline{1-2}
% 	\end{tabular}
% 	\end{subtable}

% 	\vspace*{0.5 cm}

% 	\begin{subtable}{\linewidth}
% 	\centering
% 	\caption{UADB BG=D1 \\ Similar to tuple level}
% 	\begin{tabular}{ |c|c|l}
% 				\cline{1-2}
% 		\textbf{A}  & \textbf{B}  & (c, d, p)  \\
% 		\cline{1-2}
% 		$1^{[1,1]}$ & $1^{[1,1]}$ & (2,2,3)\\
% %				\cline{1-3}
% 		$1^{[1,1]}$ & $2^{[2,2]}$ & (2,3,3)\\
% %				\cline{1-3}
% 		$2^{[2,2]}$ & $3^{[3,3]}$ & (0,1,1)\\
% 		$1^{[1,1]}$ & $3^{[3,3]}$ & (0,0,2)\\
% 				\cline{1-2}
% 	\end{tabular}
% 	\end{subtable}

% 	\vspace*{0.5 cm}

% 	\begin{subtable}{\linewidth}
% 	\centering
% 	\caption{UADB one-liner}
% 	\begin{tabular}{ |c|c|l}
% 				\cline{1-2}
% 		\textbf{A}  & \textbf{B}  & (c, d, p)  \\
% 		\cline{1-2}
% 		$1^{[1,2]}$ & $1^{[1,3]}$ & (6,6,7)\\
% %				\cline{1-3}
% 				\cline{1-2}
% 	\end{tabular}
% 	\end{subtable}

% 	\vspace*{0.5 cm}

% 	\begin{subtable}{\linewidth}
% 	\centering
% 	\caption{UADB BG=D1}
% 	\begin{tabular}{ |c|c|l}
% 				\cline{1-2}
% 		\textbf{A}  & \textbf{B}  & (c, d, p)  \\
% 		\cline{1-2}
% 		$1^{[1,1]}$ & $1^{[1,1]}$ & (2,2,3)\\
% %				\cline{1-3}
% 		$1^{[1,1]}$ & $2^{[2,3]}$ & (3,3,3)\\
% %				\cline{1-3}
% 		$2^{[1,2]}$ & $3^{[3,3]}$ & (1,1,1)\\
% 				\cline{1-2}
% 	\end{tabular}
% 	\end{subtable}

% 	\vspace*{0.5 cm}

% 	\begin{subtable}{\linewidth}
% 	\centering
% 	\caption{UADB GB=D1 tuple matchings}
% 	\begin{tabular}{ |c|}
% 				\cline{1-1}
% 		\textbf{Certain matching}\\
% 		\cline{1-1}
% 		$(1^{[1,1]}, 1^{[1,1]}) \rightarrow D1(1,1) = 2$\\
% %				\cline{1-3}
% 		$(1^{[1,1]}, 2^{[2,3]}) \rightarrow D1(1,2) = 3$\\
% %				\cline{1-3}
% 		$(2^{[1,2]}, 3^{[3,3]}) \rightarrow D1(2,3) = 1$\\
% 				\cline{1-1}
% 		$(1^{[1,1]}, 1^{[1,1]}) \rightarrow D2(1,1) = 2$\\
% %				\cline{1-3}
% 		$(1^{[1,1]}, 2^{[2,3]}) \rightarrow D2(1,2) = 2$\\
% %				\cline{1-3}
% 		$(1^{[1,1]}, 2^{[2,3]}) \rightarrow D2(1,3) = 1$\\
% 		$(2^{[1,2]}, 3^{[3,3]}) \rightarrow D2(1,3) = 1$\\
% 			\cline{1-1}
% 		\textbf{Possible matching} \\
% 		\cline{1-1}
% 		$(1^{[1,1]}, 1^{[1,1]}) \rightarrow D2(1,1) = 1$\\
% 		$(1^{[1,1]}, 1^{[1,1]}) \rightarrow D1(1,1) = 1$\\
% 		\cline{1-1}
% 	\end{tabular}
% 	\end{subtable}
% \BG{Do we need this long example here?}
% \caption{A \abbrUAADB-DB instance correspond to possible worlds semantics}
% \label{fig:exp1}
% \end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Encoding Bounds}\label{sec:uaadb-bounds}

We now define what it means for an \abbrUAADB to bound an incomplete $\semN$-relation. For that, we first define bounding of deterministic tuples by range-annotated tuples. % bound (match).
%We use \abbrUAADB relation to bound all possible worlds from an incomplete database. Starting from bounding a tuple from each possible world to a \abbrUAADB tuple.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{Definition}% [Tuple Bounding]
  \label{def:bounding-tuples}
  Let  $\rangeTup$ be a  range-annotated tuple with schema $\tuple{a_1, \ldots, a_n}$ and   $\tup$ be a tuple  with the same schema as $\rangeTup$. We say that $\rangeTup$ bounds $\tup$ written as $\tup \tmatch \rangeTup$ iff\\[-3mm]
  %
  \[
    \forall{i \in \{1, \ldots ,n\}}:
    \lbMarker{\rangeTup.a_i} \leq \tup.a_i \leq \ubMarker{\rangeTup.a_i}
  \]
\end{Definition}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{Definition}[Bounding $\uaaN$ Annotations]\label{def:bounding-annotations}
% 	A value $k \in \uaaN$ is said to bound a set of values $S_k = \{k_1, \ldots, k_n\}$ from $\semN$ if:
%   \begin{align*}
%     \forall k_i \in S_k: \lbMarker{k} \leq k_i \leq \ubMarker{k}\\
%     \exists k_i \in S_k: k_i = \bgMarker{k}
%   \end{align*}
% \end{Definition}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

One \abbrUAADB tuple may bound multiple conventional tuples and vice versa. We define \textit{tuple matchings} as a way to match the multiplicities of  tuples of a $\uaaN$-database (or relation) with that of one possible world of an incomplete $\semN$-database (or relation).
Based on tuple matchings we then define how to  bound possible worlds.
% a mapping between a set of \abbrUAADB tuples and a set of deterministic tuples.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{Definition}% [Tuple matching]
  \label{def:tuple-matching}
  Let $\rangeRel$ be an $n$-ary \abbrUAARel and $\rela$ an $n$-ary relation. A \emph{tuple matching} $\TM$ for $\rangeRel$ and $\rela$ is a function $(\rangeDom)^{n} \times \dataDomain^n \to \semN$.
  % $$TM_{R^I,R}(\rangeTup,t)=k$$ is the mappings from an annotated tuple $\rangeTup$ and a possible world tuple $t$ to a semiring element $k$
  \st the following conditions hold:\\[-3mm]
  %%%%%%%%%%%%%%%%%%%%
  \begin{align*}
    &\forall \rangeTup \in \rangeDom^n: \forall \tup \ntmatch \rangeTup: \TM(\rangeTup, \tup) = \zeroN
    &\forall \tup \in \dataDomain^n: \hspace*{-1mm}\sum_{\rangeTup \in \rangeDom^n} \hspace*{-1mm}\TM(\rangeTup, \tup)=\rela(\tup)
  \end{align*}
\end{Definition}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

A tuple matching distributes the multiplicity of a tuple from $\rela$ over one or more matching tuples from $\rangeRel$.  Multiple tuples from an \abbrUAADB may encode the same tuple when the multidimensional rectangles of their attribute-level range annotations overlap, as with the first two tuples of the \abbrUAADB in \Cref{table:UAAR_overall} and the \abbrBGW.
%. For instance,  $\tuple{\uv{1}{2}{3}}$ and $\tuple{\uv{2}{3}{5}}$ both match the tuple $\tuple{2}$.
% The conditions stating that a \abbrUAADB tuple can only match to conventional tuple if the tuple is bounded by the \abbrUAADB tuple. Also all the conventional tuples in relation $\rela$ need to be matched in the tuple matching.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{Definition}\label{def:bounding-worlds}
  Given an n-ary \abbrUAADB relation $\rangeRel$ and an n-ary deterministic $\semN$-relation $\rela$ (a possible world),  relation $\rangeRel$ bounds $\rela$ (denoted $\rela \dbbounds \rangeRel$) iff there exists a tuple matching $\TM$ for $\rangeRel$ and $\rela$ \st \\[-5mm]
%
  \begin{align*} %\label{eq:lower-bound-db}
    &\forall \rangeTup \in \rangeDom^n:\sum_{\tup \in \dataDomain^n} \TM(\rangeTup,\tup) \geq \lbMarker{\rangeRel(\rangeTup)}
    \;\text{\textbf{and}}\; % \forall \rangeTup \in \rangeDom^n:
       \sum_{\tup \in \dataDomain^n} \TM(\rangeTup,\tup) \leq \ubMarker{\rangeRel(\rangeTup)} %\label{eq:upper-bound-db}
  \end{align*}
\end{Definition}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Having defined when a possible world is bound by a $\uaaN$-relation, we are ready to define bounding of incomplete $\semN$-relations.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{Definition}\label{def:bounding-incomplete-dbs}
	Given an incomplete $\semN$-relation $\prel$ and a $\uaaN$-relation $\rangeRel$, we say that $\rangeRel$ bounds $\prel$, written as $\prel \dbbounds \rangeRel$
  iff
    \begin{align*}
    &\forall \rela \in \prel: \rela \dbbounds \rangeRel
    &&\exists \rela \in \prel: \rela = \bgOf{\rangeRel}
    \end{align*}
\end{Definition}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\noindent These definitions are extended to databases in the obvious way.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{Example}\label{ex:bounding-incomplete-dbs}
  Consider the \abbrUAADB of \Cref{ex:audb-instance} and the worlds of~\Cref{table:UAAR_bg}. % shown below.
%
%   \begin{minipage}{0.49\linewidth}
%     \centering
%     \underline{$\db_1$}                                                                           \\
%     	\begin{tabular}{lc|cc}
%                                & \textbf{A}                 & \textbf{B} & \underline{$\semN$}    \\
% 		\cline{2-3}
% $\tup_1$                       & $1$                        & $1$        & 5                      \\
% $\tup_2$                       & $2$                        & $3$        & 1                      \\
% 	\end{tabular}
%   \end{minipage}
%   \begin{minipage}{0.49\linewidth}
%     \centering
%     \underline{$\db_2$}                                                                           \\
%     \begin{tabular}{lc|cc}
%                                & \textbf{A}                 & \textbf{B} & \underline{$\semN$}    \\
% 		\cline{2-3}
%  $\tup_3$                      & $1$                        & $1$        & 2                      \\
%  $\tup_4$                      & 1                          & 3          & 2                      \\
% $\tup_5$                       & $2$                        & $4$        & 1                      \\
% 	\end{tabular}
%   \end{minipage}
  The \abbrUAADB bounds these worlds, since there exist tuple matchings that provide a lower and an upper bound for the annotations of the tuples of each world. For instance, denoting the tuples from this example as
  %
  \begin{align*}
    \rangeTup_1                & \defas \tuple{\uv{1}{1}{1}, \uv{1}{1}{1}}
                               & \rangeTup_2                & \defas \tuple{\uv{1}{1}{1}, \uv{1}{1}{3}}\\
                                \rangeTup_3                & \defas \tuple{\uv{1}{2}{2}, \uv{3}{3}{3}}
  \end{align*} %
  \iftechreport{Tuple matchings $\TM_1$ and $\TM_2$ shown below to bound $\db_1$ and $\db_2$.}
  \ifnottechreport{Tuple matching $\TM_1$ (shown below) bounds $\db_1$.}
  \begin{align*}
    \TM_1(\rangeTup_1, \tup_1) & = 2
                               & \TM_1(\rangeTup_2, \tup_1) & = 3
                               & \TM_1(\rangeTup_3, \tup_1) & = 0                                 \\
    \TM_1(\rangeTup_1, \tup_2) & = 0
                               & \TM_1(\rangeTup_2, \tup_2) & = 0
                               & \TM_1(\rangeTup_3, \tup_2) & = 1
    \iftechreport{\\[2mm]
    \TM_2(\rangeTup_1, \tup_3) & = 2
                               & \TM_2(\rangeTup_2, \tup_3) & = 0
                               & \TM_2(\rangeTup_3, \tup_3) & = 0                                 \\
    \TM_2(\rangeTup_1, \tup_4) & = 0
                               & \TM_2(\rangeTup_2, \tup_4) & = 2
                               & \TM_2(\rangeTup_3, \tup_4) & = 0                                 \\
    \TM_2(\rangeTup_1, \tup_5) & = 0
                               & \TM_2(\rangeTup_2, \tup_5) & = 0
                               & \TM_2(\rangeTup_3, \tup_5) & = 1
%
}
  \end{align*}
    \end{Example}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \BG{removed this: fig:exp1 shows an example of a \abbrUAADB-DB with a possible tuple matching that fulfills the correctness criteria.}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Tightness of Bounds}
\label{sec:approximation-factor}

% \Cref{def:bounding-incomplete-dbs} defines what it means for an \abbrUAADB to bound an incomplete databases. However,
Given an incomplete database, there are many possible \abbrUAADBs that bound it of varying tightness. For instance, both $\rangeTup_1 \defas \tuple{\uv{1}{15}{100}}$ and $\rangeTup_2 \defas \tuple{\uv{13}{14}{15}}$ bound tuple $\tuple{15}$, but intuitively the bounds provided by $\rangeTup_2$ are tighter. We develop a metric for the tightness of the approximation provided by an \abbrUAADB and prove that finding an \abbrUAADB that maximizes tightness % when we limit the size of the \abbrUAADB
is intractable. Given two \abbrUAADBs $\rangeDB$ and $\rangeDB'$ that both bound an incomplete $\semN$-database $\pdb$, $\rangeDB$ is a tighter bound than $\rangeDB'$ if the set of worlds bound by $\rangeDB$ is a subset of the set of worlds bound by $\rangeDB'$. % As a sanity check, consider $\rangeDB_1 \defas \{t_1\}$ and $\rangeDB_2 \defas \{t_2\}$ using $t_1$ and $t_2$ from above and assume that $\dataDomain = \semN$. Then $\rangeDB_2$ is a tighter bound than $\rangeDB_1$ since the three deterministic databases it bounds $\{(13)\}$, $\{(14)\}$ and $\{(15)\}$ are also bound by $\rangeDB_1$, but $\rangeDB_1$ bounds additional databases, e.g., $\{(2)\}$. % that are not bound by $\rangeDB_2$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{Definition}% [Bound Tightness]
  \label{def:bound-tightness}
  Consider two $\uaaN$-databases $\rangeDB$ and $\rangeDB'$ over the same schema
$\aschema$. We say that $\rangeDB$ is at least as tight as $\rangeDB'$, written as $\rangeDB \dbleq \rangeDB'$, if for all $\semN$-databases $\db$ with schema $\aschema$ we have:
  \begin{align*}
 \db \dbbounds \rangeDB \rightarrow \db \dbbounds \rangeDB'
  \end{align*}
  We say that $\rangeDB$ is strictly tighter than $\rangeDB'$, written as $\rangeDB \dble \rangeDB'$ if $\rangeDB \dbleq \rangeDB'$ and there exists $\db \dbbounds \rangeDB'$ with $\db \not\dbbounds \rangeDB$. Furthermore, we call $\rangeDB$  a maximally tight bound for an incomplete $\semN$-database $\pdb$ if:
  \begin{align*}
    \pdb &\dbbounds \rangeDB
   &\not \exists \rangeDB':\; \pdb \dbbounds \rangeDB' \wedge \rangeDB' \dble \rangeDB
  \end{align*}
\end{Definition}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

This notion of tightness is well-defined even if the data domain $\dataDomain$ is infinite. % For instance, if we use the reals $\mathbb{R}$ instead of natural numbers as the domain in the example above, then still $\rangeDB_1 \dbge \rangeDB_2$.
In general \abbrUAADBs that are tighter bounds are preferable. However, computing a maximally tight bound is intractable.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{Theorem}\label{def:intractability-of-tight-bounds}
Let $\pdb$ be an incomplete $\semN$-database encoded as a \abbrCtable~\cite{DBLP:journals/jacm/ImielinskiL84}.  % in the size of $\pdb$
Computing a maximally tight bound $\rangeDB$ for $\pdb$ is \nphard.
\end{Theorem}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{proof}[Proof Sketch]
  \ifnottechreport{
    Proven by reduction from 3-colorability~\cite{techreport}.
    We construct a C-table with one tuple and encode the 3-colorability of the input graph $G$ in the local condition of the tuple, i.e., the tuple is possible iff $G$ is 3-colorable.
    The maximally tight  upper multiplicity bound for this tuple is $1$ iff graph $G$ is 3-colorable.
  }
  \iftechreport{
We prove the claim through a reduction from 3-colorability.
\BG{Write proof. can we generalize to any model not just C-tables. If yes, does this require a size-bound?}
    }
\end{proof}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%In the light of this result, we devise methods for translating incomplete and probabilistic databases into \abbrUAADBs that do not guarantee tight bounds.
% Even if we were able to compute tight bounds, preserving these bounds under  queries is computationally hard. This follows from well-known hardness results for computing certain answers.
% Thus, % even if the input is maximally tight,
% our query semantics does not preserve tightness of bounds.
% Note that this strictly necessary since computing tight bounds on aggregation function results is already hard in incomplete and probabilistic databases (e.g., see~\cite{DBLP:journals/tcs/ArenasBCHRS03}).
% Nonetheless, % comparing the tightness of \abbrUAADBs is useful for
% we will use this metric in \Cref{sec:experiments} to evaluate relative tightness of bounds.
  % (this follows from hardness results for computing tight bounds for the results of an aggregation query over incomplete databases).
%\subsection{Tuple matching}
%Define matching $t' \tmatches t$ as true iff $\forall{i \in [1,n]}:t(a_i) \in I_{t'(a_i)}$ \\
%A tuple matching $TM_{R',R}(t',t)=k$ is the mappings from an annotated tuple $t'$ and a possible world tuple $t$ to a semiring value $k$. \\
%As a constrain, any tuple matching need to fully match all certain tuples from annotated relation:
%$$\forall_{t' \in R'}:\sum_{t \in R}TM_{R',R}(t',t)=R'(t').k_c$$
%A annotated relation $R'$ is c-sound if:
%$$\forall_{D(R) \in \dataDomain}:\exists TM_{R',R}:\forall_{t \in R}:\sum_{t' \in R'}TM_{R',R}(t',t) \leq R(t)$$
%A annotated relation $R'$ is p-complete if:
%$$\forall_{t' \in R'}:\sum_{t \in R}TM_{R',R}(t',t)=R'(t').k_p$$
%$$\forall_{D(R) \in \dataDomain}:\exists TM_{R',R}:\forall_{t \in R}:\sum_{t' \in R'}TM_{R',R}(t',t) \geq R(t)$$



%%%
%\subsection{Certain tuples based tuple matching}
%In certain tuples based tuple matching, we match annotated tuples to certain tuples in all possible worlds.\\
%An annotated relation $R'$ is c-sound if:
%$$\exists TM:\forall_{t' \in R'}:\sum_{t \in R}TM(R',R,t',t) \leq certain(\dataDomain)(t)$$
%A annotated relation $R'$ is c-complete if:
%$$\exists TM:\forall_{t' \in R'}:\sum_{t \in R}TM(R',R,t',t) \geq certain(\dataDomain)(t)$$
%%%

%\subsection{Expressions}
%An attribute $x$ is certain iff the upper bound and lower bound of the attribute are equal.
%Comparison and boolean operators can be defined as:
%\begin{enumerate}
%\item \[ \begin{cases}
%\ubMarker{(a>b)} = T & \text{if } \ubMarker{a}>\lbMarker{b} \\
%\ubMarker{(a>b)} = \bfalse & \text{else}
%\end{cases}
%\]
%\[ \begin{cases}
%\lbMarker{(a>b)} = T & \text{if } \lbMarker{a}>\ubMarker{b} \\
%\lbMarker{(a>b)} = \bfalse & \text{else}
%\end{cases}
%\]
%\item \[ \begin{cases}
%\ubMarker{(a=b)} = T & \text{if } \ubMarker{a}>\lbMarker{b} \wedge \lbMarker{a}<\lbMarker{b} \vee \ubMarker{a}>\ubMarker{b} \wedge \lbMarker{a}<\ubMarker{b} \\
%\ubMarker{(a=b)} = \bfalse & \text{else}
%\end{cases}
%\]
%\[
%\begin{cases}
%\lbMarker{(a=b)} = \btrue & \text{if } \ubMarker{a}=\lbMarker{b} \wedge \ubMarker{b}=\lbMarker{a} \\
%\lbMarker{(a=b)} = \bfalse & \text{else}
%\end{cases}
%\]
%\item \[ \ubMarker{(p \wedge q)} = \ubMarker{p} \wedge \ubMarker{q} \]
%\[ \lbMarker{(p \wedge q)} = \lbMarker{p} \wedge \lbMarker{q} \]
%\item \[ \ubMarker{(p \vee q)} = \ubMarker{p} \vee \ubMarker{q} \]
%\[ \lbMarker{(p \vee q)} = \lbMarker{p} \vee \lbMarker{q} \]
%\end{enumerate}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "uaadb"
%%% End:

